Confidence-Based Feature Imputation for Graphs with Partially Known Features

This paper investigates a missing feature imputation problem for graph learning tasks. Several methods have previously addressed learning tasks on graphs with missing features. However, in cases of high rates of missing features, they were unable to avoid significant performance degradation. To overcome this limitation, we introduce a novel concept of channel-wise confidence in a node feature, which is assigned to each imputed channel feature of a node for reflecting certainty of the imputation. We then design pseudo-confidence using the channel-wise shortest path distance between a missing-feature node and its nearest known-feature node to replace unavailable true confidence in an actual learning process. Based on the pseudo-confidence, we propose a novel feature imputation scheme that performs channel-wise inter-node diffusion and node-wise inter-channel propagation. The scheme can endure even at an exceedingly high missing rate (e.g., 99.5\%) and it achieves state-of-the-art accuracy for both semi-supervised node classification and link prediction on various datasets containing a high rate of missing features. Codes are available at https://github.com/daehoum1/pcfi.

==> Neurips_2022/0-Abstract_0.tex <==
\begin{abstract}

In this paper, we tackle a missing feature recovery problem for \rv{graph learning tasks}. Since existing methods recover the missing features based on only inter-node diffusion via edges of a graph, they could not effectively handle channel-wise missing features. To overcome this limitation, we introduce a novel concept of channel-wise confidence in a node feature, which is assigned to each recovered channel feature of a node for reflecting certainty of the recovery. To replace unavailable true confidence in an actual learning process, we design a pseudo-confidence by using the channel-wise shortest path distance between a missing-feature node and its nearest known-feature node. Based on the pseudo-confidence, we propose a novel feature recovery scheme that performs both channel-wise graph diffusion and node-wise inter-channel propagation in contrast to existing methods. The scheme can endure even at a very high missing rate (e.g., 99.5\%) and achieves state-of-the-art accuracy for \rv{both semi-supervised node classification and link prediction} on various datasets containing a high rate of missing features.


\end{abstract}


==> Neurips_2022/1-Intro_2.tex <==
\section{Introduction}
\vspace{-0.4mm}
\label{Intro}
In recent years, graph neural networks (GNNs) have received a lot of attention and have shown outstanding performance on numerous problems in various fields~\cite{zhou2020graph, wu2020comprehensive, zhang2020deep,zitnik2018modeling,ying2018graph, yan2018spatial, fout2017protein}. \rv{While various GNNs are designed for node representation learning~\cite{velivckovic2017graph, xu2018representation, kipf2016semi, defferrard2016convolutional} and graph representation learning~\cite{kipf2016variational, sun2019infograph, velickovic2019deep},} GNN models typically assume that features for all nodes are fully observed. However, in real-world situations, features in graph-structured data are often partially observed as illustrated in the following cases. First, collecting complete data for a large graph is expensive or even impossible. Secondly, in social networks, most users want to protect their personal information selectively. Besides, \rv{measurement failure often occurs or there can exist newly joined nodes after measurement.} Under these situations, most GNNs cannot be directly applied due to incomplete features.

Several methods have been proposed to handle missing features \cite{taguchi2021graph,jiang2020incomplete,monti2017geometric,rossi2021unreasonable}, but they suffer from significant performance degradation at \rv{very} high rates of missing features. Feature Propagation (FP)~\cite{rossi2021unreasonable}, which iteratively propagates known features among the nodes, 
shows improved performance but still cannot avoid a considerable accuracy drop at a high missing rate. 
%which recovers missing features by inter-node propagation of known features via edges in a graph. to the nodes  through edges the nodes,
In real-world scenarios, extremely sparse data~\cite{ref:wind_data, ref:extreme_sparse_18} commonly exist, which is significant but challenging.

To fully exploit the sparsely-known channel feature in each node, in this paper, we design an elaborate feature recovery scheme that diffuses the known features with different intensities per channel, unlike the inter-node diffusion used in FP.
To this end, we \rv{devise} two schemes for both channel-wise and node-wise feature recovery, called channel-wise graph diffusion and node-wise inter-channel propagation.
%While FP diffuses features only among nodes, to fully exploit the sparse known feature, we consider propagation among channel features inside each node containing sparsely-known channel feature, i.e.,
%node-wise Inter-channel propagation (NwIcP). To design NwIcP, the connectivity between channel features should be defined in each node. Also, we consider channel-wise Inter-node diffusion (CwInD) to leverage the graph structure.
To assign the diffusion intensity per channel in every node,
%of each feature value for both CwInD and NwIcP, 
we introduce a novel concept of channel-wise confidence
%in each feature value,
which reflects the quality of channel feature recovery.
%after learning. 

The true confidence in missing channel feature is not accessible before recovery. Thus we propose pseudo-confidence to be used in our recovery scheme instead of true confidence. %Since channel-wise confidence is not accessible value in the learning process, we calculate channel-wise pseudo-confidence (PC) which leverages the channel-wise shortest path distance from a missing-feature node to its nearest known-feature node.
%PC plays a key role in determining the degree of message passing in both CwInD and NwIcP. 
By using channel-wise confidence in our scheme, the less confident channel feature can be recovered by aggregating the highly confident channel features in each node or by highly confident channel features diffused from neighboring nodes.  
%according to the importance of each channel value. Moreover, since channel-wise confidence also differs across the nodes, feature for update can aggregate features from connected nodes according to the importance of each feature value.

The key contribution of our work can be summarized as follows: (1) We propose a new concept of channel-wise confidence that represents the quality of a recovered channel feature.
(2) We design a method to give pseudo-confidence that can be used instead of unavailable true confidence in a missing channel feature.
(3) Based on the pseudo-confidence, we propose a novel feature recovery scheme which achieves the state-of-the-art \rv{performance} for \rv{node classification and link prediction} even in a very high missing rate (e.g., 99.5\%) of missing features.

\vspace{-0.6mm}

==> Neurips_2022/2-Related_0.tex <==
\section{Related Work}
\label{Related}

\vspace{-0.3mm}
\subsection{Learning on Graphs with Missing Node Features}
\vspace{-0.3mm}

\rv{The problem of missing data has been widely studied in the literature~\cite{little2019statistical, loh2011high, you2020handling, zhang2022non, najafi2022missing, gordon2021tsi}.} Recently, \rv{focusing on graph-structured data}, there have been several attempts to learn graphs with missing node features. Monti et el.~\cite{monti2017geometric} proposed recurrent multi-graph convolutional neural networks (RMGCNN) and separable RMGCNN(sRMGCNN), a scalable version of RMGCNN. Both of them combine a multi-graph convolutional neural network and LSTM~\cite{hochreiter1997long} for matrix completion on multi-graphs. Structure-attribute transformer (SAT)~\cite{chen2020learning} models the joint distribution of graph structures and node attributes by distribution techniques, then completes missing node attributes. GCN for missing features (GCNMF)~\cite{taguchi2021graph} adapts graph convolutional networks (GCN)~\cite{kipf2016semi} to graphs that contain missing node features via representing the missing features by Gaussian mixture model. Meanwhile, a partial graph neural network (PaGNN)~\cite{jiang2020incomplete} leverages a partial message-propagation scheme that considers only known features during propagation. However, these methods suffer large performance degradation when there exists a high feature missing rate. Feature propagation (FP)~\cite{rossi2021unreasonable} reconstructs missing features by diffusing known features. However, in diffusion of FP, a missing feature is formed by aggregating features from neighboring nodes regardless of whether a feature is known or inferred. Moreover, FP does not consider any interdependency among feature channels. To utilize relationships among channels, we construct a covariance matrix of pre-recovered features and update features additionally.

\vspace{-0.3mm}
\subsection{Distance Encoding}
\vspace{-0.3mm}

Distance encoding (DE) on graphs defines extra features by using distance from a node to the node set where the prediction is to be made. Zhang and Chen~\cite{zhang2018link} extracts a local enclosing subgraph around each target node pair, and uses GNN to learn graph structure features for link prediction. Li et al.~\cite{li2020distance} exploits structure-related features termed DE that encodes distance between a node and its neighboring node set by graph-distance measures (e.g., shortest path distance or generalized PageRank scores~\cite{li2019optimizing}). Zhang et al.~\cite{zhang2021labeling} unifies the aforementioned techniques into \textit{labeling trick}. Heterogeneous graph neural network (HGNN)~\cite{ji2021heterogeneous} proposes a heterogeneous distance encoding in consideration of multiple types of paths in enclosing subgraphs of heterogeneous graphs. Distance encoding in existing methods improves the representation power of GNNs. We use distance encoding to distinguish missing features based on the shortest path distance from a missing feature to known features in the same channel.

\vspace{-0.3mm}
\subsection{Graph Diffusion}
\vspace{-0.3mm}
Diffusion on graphs spreads the feature of each node to its neighboring nodes along the edges.~\cite{coifman2006diffusion, shuman2013emerging, guille2013information}. There are two types of transition matrices commonly used for diffusion on graphs: symmetric transition matrix~\cite{kipf2016semi, klicpera2019diffusion, rossi2021unreasonable} and random walk matrix~\cite{page1999pagerank, chung2007heat, perozzi2014deepwalk, grover2016node2vec, atwood2016diffusion, klicpera2018predict, lim2021class}. While these matrices work well for each target task, from a node's point of view, the sum of edge weights for aggregating features is not $1$ in general. Therefore, since features are not updated at the same scale of original features, these matrices are not suitable for missing feature recovery. 


==> Neurips_2022/3-Proposed_0.tex <==
\section{Proposed Method}
\label{Proposed}
\vspace{-0.2mm}
\input{3.1-3}
\vspace{-0.2mm}
\input{3.3-3}
\vspace{-0.2mm}
\input{3.2-2}
\vspace{-0.2mm}
%\input{3.3-3}
\input{3.4-2}
\vspace{-0.2mm}
\input{3.5-2}

==> Neurips_2022/3.1-3.tex <==
\subsection{Overview}
\label{problem_statement}
\input{figure-framework}
\vspace{-0.7mm}
In our work, we tackle a problem for
\textbf{\rv{graph learning tasks with missing node features}.} 
The \rv{first} target task\rv{, semi-supervised node classification,} is to infer the labels of the remaining unlabeled/missing feature nodes from the partially known features/labels and the fully known graph structure. \rv{The second target task, link prediction, is to predict whether two nodes are likely to have a link.}
Figure~\ref{fig:framework} depicts overall scheme of the proposed feature recovery scheme to 
address \rv{graph learning tasks with missing features}.
Our key idea is to recover the missing feature in a channel-wise manner.
To this end, we devise two feature recovery stages: channel-wise graph diffusion and node-wise inter-channel propagation.
The recovered features are used for \rv{downstream tasks} via an off-the-shelf GNNs. 

%Our feature recovery scheme is based on channel-wise confidence defined on each channel feature of every node. Instead of unavailable true confidence, we use a pseudo-confidence of a recovered feature in a missing node, which is designed using the graph structure and partially known features. 


In Sec.~\ref{sub:notations}, we first introduce the notations used in this paper.
In Sec.~\ref{sub:ecfr}, we give an outline of the proposed PC (pseudo-confidence)-based feature recovery (PCFR) scheme which recovers missing node features. 
We then propose a method to determine the \textit{pseudo-confidence} in Sec.~\ref{sub:confidence}. In Sec.~\ref{sub:ecfd} we present channel-wise graph diffusion that iteratively propagates known features in consideration of PC. In Sec.~\ref{sub:ccp}, we present node-wise inter-channel propagation which adjusts features based on covariance between channels.
\vspace{-0.4mm}




\subsection{Notations}
\label{sub:notations}
\vspace{-0.3mm}
%Before explaining the problem, we begin with basic notation on graphs.

\textbf{Basic notation on graphs.} An undirected connected graph is represented as $\mathcal{G} = (\mathcal{V}, \mathcal{E}, A)$ where $\mathcal{V}=\{v_i\}^N _{i=1}$ is the set of $N$ nodes, $\mathcal{E}$ is the edge set with $(v_i, v_j) \in \mathcal{E}$, and $A \in \{0,1\}^{N \times N}$ denotes an adjacency matrix. $X = [x_{i,d}] \in \mathbb{R}^{N \times F}$ is a $F$-channel node feature matrix, i.e., $x_{i,d}$, the $d$-th channel value of the node $v_i$. $\mathcal{N}(v_i)$ denotes the set of neighbors of $v_i$. Given an arbitrary matrix $M \in \mathbb{R}^{n \times m}$, we let $M_{i, :}$ denote the $i$-th row vector of $M$. Similarly, we let $M_{:, j}$ denote the $j$-th column vector of $M$.

\textbf{Notation for graphs with missing node features.} As we assume partial or even very few node features are known, we define $\mathcal{V}^{(d)}_k$ as the set of nodes where the $d$-th channel feature values are known ($k$ in $\mathcal{V}^{(d)}_k$ means `known'). The set of nodes with the unknown $d$-th channel feature values is denoted by
$\mathcal{V}^{(d)}_u = \mathcal{V} \setminus \mathcal{V}^{(d)}_k$. Then $\mathcal{V}^{(d)}_k$ and $\mathcal{V}^{(d)}_u$ are referred to source nodes and missing nodes, respectively. By reordering the nodes according to whether a feature value is known or not for the $d$-th channel, we can write graph signal for the $d$-th channel features and adjacency matrix as
\begin{equation*}
x^{(d)}=
\begin{bmatrix}
x^{(d)}_k\\
x^{(d)}_u
\end{bmatrix}
\qquad
A^{(d)} =
\begin{bmatrix}
A^{(d)}_{kk} & A^{(d)}_{ku} \\
A^{(d)}_{uk} & A^{(d)}_{uu}
\end{bmatrix}.
\end{equation*}
Here, $x^{(d)}$, $x^{(d)}_k$, and $x^{(d)}_u$ are column vectors that represent corresponding graph signal. Since the graph is undirected, $A^{(d)}$ is symmetric and thus $(A^{(d)}_{ku})^\top = A^{(d)}_{uk}$. Note that $A^{(d)}$ is different from $A$ due to reordering while they represent the same graph structure. \rv{$\tilde{X} = [ \tilde{x}_{i,d}]$} denotes recovered features for $X$ from $\{x^{(d)}_k\}^F_{d=1}$ and $\{A^{(d)}\}^F_{d=1}$.
A summary of notations is in Table \ref{notation_table}.
\input{tables/notation_table}
 


==> Neurips_2022/3.2-2.tex <==
\subsection{Pseudo-Confidence}
\label{sub:confidence}
\vspace{-0.4mm}
%Our goal is to recover missing features from the given features of all source nodes in $\mathcal{G}$. To this end, we introduce a new concept, confidence on a recovered feature in a node.
We first define the concept of confidence in the recovered feature $\hat{x}_{i,d}$ of a node $v_i$ for channel $d$.
\begin{definition} \label{definition1}
Confidence in the recovered channel feature $\hat{x}_{i,d}$ is defined by similarity between $\hat{x}_{i,d}$ and true one $x_{i,d}$, which is a value between 0 and 1.
\end{definition}
Note that the feature $x_{i,d}$ of a source node is fully observed and thus its confidence becomes 1. When the recovered  $\hat{x}_{i,d}$ is far from the true  ${x}_{i,d}$, the confidence in $\hat{x}_{i,d}$ will decrease towards 0. 
% However, the recovered feature $\hat{x}_{i,d}$ of a missing node should be obtained by using the confidence in our work, whereas the confidence can not be calculated before getting $\hat{x}_{i,d}$. 
%However, when we try to use the confidence to recover $x_{i,d}$ in practice, true value $x_{i,d}$ is not accessible value due to missing. Moreover, we cannot infer $\hat{x}_{i,d}$ before any learning.
However, it is a chicken and egg problem to find $\hat{x}_{i,d}$ and its confidence. That is, the confidence in $\hat{x}_{i,d}$ is unavailable before getting $\hat{x}_{i,d}$ according to Definition \ref{definition1}, whereas the proposed scheme can not yield $\hat{x}_{i,d}$ without the confidence. 

To handle this issue, instead of true confidence, we design the pseudo-confidence by using shortest path distance between a node and its nearest source node for a specific channel (SPD-S). 
For instance, 
SPD-S of the $i$-th node for the $d$-th channel feature is denoted by $S_{i,d}$ which is calculated by \begin{equation}
\label{eq:SPDS}
S_{i,d}=s(v_i|\mathcal{V}^{(d)}_k, A^{(d)}),
\end{equation}
where $s(\cdot)$ yields the shortest path distance between the $i$-th node and its nearest source node 
in $\mathcal{V}^{(d)}_k$ on $A^{(d)}$. Note that if the $i$-th node is a source node, its nearest source node is itself, thus $S_{i,d}$ becomes zero.
We construct SPD-S matrix $S \in \mathbb{R}^{N \times F}$ of which elements are $S_{i,d}$.

Consider $\hat{X}=[\hat{X}_{i,d}]$ that represents the recovered features of $X$ with consideration of feature homophily\rv{~\cite{mcpherson2001birds}} that is a local property on a graph~\cite{bisgin2010investigating, lauw2010homophily, bisgin2012study}. Based on the feature homophily, the feature similarity between any two nodes tends to increase as the shortest path distance between the two nodes decreases.
Hence the recovered 
feature $\hat{x}_{i,d}$ of a node $v_i$ becomes similar to the given feature of its nearest source node more confidently as SPD-S  of $v_i$ ($S_{i,d}$) decreases.

Based on this homophily, we define the pseudo-confidence using SPD-S in Definition \ref{definition2}.


\begin{definition}
\label{definition2}
Pseudo-confidence (PC) in $\hat{x}_{i,d}$ is defined by a function  ${\rho}_{i,d}
%(\hat{x}_{i,d}|\mathcal{V}^{d}_k , A^{(d)})
= \alpha^{S_{i,d}}$ where $\alpha \in (0, 1)$ is a hyperparameter.
\end{definition}
By Definition \ref{definition2}, PC becomes 1 for $\hat{x}_{i,d}={x}_{i,d}$ on source nodes. Also, PC for a missing node features decreases exponentially as $S_{i,d}$ increases. Likewise, PC reflects well the tendency of confidence in Definition \ref{definition1}.



==> Neurips_2022/3.3-3.tex <==
%\input{figure-framework}
\subsection{PC-based Feature Recovery Scheme }
\vspace{-0.3mm}
\label{sub:ecfr}
The proposed PC-based feature recovery (PCFR) scheme leverages the shortest path distance between nodes to compute pseudo-confidence. PCFR consists of two stages: channel-wise graph diffusion and node-wise inter-channel propagation. The first stage finds $\tilde{X}$ (pre-recovered features for $X$) through PC-based feature diffusion on a given graph $\mathcal{G}$. Then, the second stage updates $\tilde{X}$ to the final recovered features $\hat{X}$ by considering both PC and correlation between channels. 

\vspace{-0.1mm}
To perform node classification \rv{and link prediction}, a GNN is trained with recovered node features $\hat{X}$. \rv{In this work, PCFR is designed to perform the downstream tasks well.} However, since PCFR is independent of the type of learning task, PCFR is not limited to the two tasks and so can be applied to various graph learning tasks with missing node features.

\vspace{-0.1mm}
Formally, the proposed framework can be expressed as
\begin{subequations}
\begin{align}
\hat{X} &= f(\{x^{(d)}_k\}^F_{d=1} ,  \{A^{(d)}\}^F_{d=1})\\
\hat{Y} &= g_\theta (\hat{X},A)\rv{,}
\end{align}
\end{subequations}
where $f$ is PCFR and $\hat{Y}$ is a prediction for desired output of a given task. Here, any GNN architecture can be adopted as $g_\theta$ according to the type of task.


==> Neurips_2022/3.4-2.tex <==
\subsection{Channel-wise Graph Diffusion}
\label{sub:ecfd}
\vspace{-0.4mm}
% In this section, we present EC-based feature diffusion which is a first stage of CBFR.

% Diffusion is a process that consists of iterative propagation, which can be expressed as iteratively multiplying a feature matrix by a transition matrix.

To recover missing node features via graph diffusion, source nodes propagate their features to their neighbors for each channel independently. While source nodes keep their features that are true values, missing nodes aggregate features from connected nodes. Missing nodes aggregate low-confidence features from other connected missing nodes in addition to high-confidence features from source nodes. Based on confidence which is an essential concept for missing feature setting, we design a novel transition matrix for feature diffusion. Our design objective is that a missing node aggregates more features of high-PC nodes. To this end, we consider PC in features for neighboring nodes of a specific missing feature.

\rv{We define relative PC that represents an amount of PC in a particular node feature relative to other node features as follows.
%\newtheorem{definition5}{Definition}
%\label{definition4}
\begin{definition}
\label{definition3}
Relative PC of $\hat{x}_{j,d}$ relative to $\hat{x}_{i,d}$ is defined by ${\rho}_{j/i,d} %(\bar{x}_{j,d}| \bar{x}_{i,d}) 
= {\rho}_{j,d} / {\rho}_{i,d}=\alpha^{S_{j,d}-S_{i,d}}$.
\end{definition}}

\rv{Then, suppose a missing node feature $x_{i,d}$ of $v_i$ aggregates features from $v_j \in \mathcal{N}(v_i)$. We observe that at the point of view of a missing node, there are only three possible cases for relative PC in its neighboring feature relative to its feature, while two cases for a source node. Formally, from the observation, we relative PCs depending on the above cases are  determined by {\bf Proposition 1} as}
\rv{
\begin{proposition}
\label{proposition1}
If $S_{i,d}=m\geq1$, then $\rho_{j/i,d} \in \{\alpha^{-1}, 1, \alpha\}\,$ for $v_j \in \mathcal{N}(v_i)$. Otherwise, if $S_{i,d}=0$, then $\rho_{j/i,d} \in \{ 1, \alpha\}\,$ for $v_j \in \mathcal{N}(v_i)$.
\end{proposition}}
The proof of {\bf Proposition 1} is given in the supplementary material. 

% Suppose a missing node feature $x_{i,d}$ of $v_i$ aggregates features from $v_j \in \mathcal{N}(v_i)$. We observe that difference between SPD-S of $v_i$ and SPD-S of $v_j$ cannot exceed 1. Formally, this observation can be expressed as the following theorem with proof in the supplementary material. 
% % \newtheorem{theorem}
% % \label{theorem1}
% \begin{theorem}
% \label{theorem1}
% Given a node $v_i$ s.t. $S_{i,d}=m\geq1$. Then, $S_{j,d} \in \{m-1,m,m+1\}$ for $v_j \in \mathcal{N}(v_i).$ Otherwise, if $v_i$ s.t. $S_{i,d}=0$ is given, $S_{j,d} \in \{0,1\}$ for $v_j \in \mathcal{N}(v_i).$
% \end{theorem}
% From Theorem \ref{theorem1}, the following corollary holds trivially.

% \begin{corollary}
% \label{corollary1}
% If $S_{i,d}=m\geq1$, then \ $S_{j,d}-S_{i,d}  \in \{-1,0,1\}$ for $v_j \in \mathcal{N}(v_i)$. Otherwise, if $S_{i,d}=0$, then $S_{j,d}-S_{i,d}  \in \{0,1\}$ for $v_j \in \mathcal{N}(v_i)$.
% \end{corollary}

% Theorem \ref{theorem1} shows that from any node, there are at most three possible cases for SPD-S of its neighbors. Further, Corollary~\ref{corollary1} shows that when moving to a neighboring node, there are at most three possible changes in SPD-S. We then define relative PC, a function to output relative amount of PC in a particular node feature compared to other node features as follows.
% %\newtheorem{definition5}{Definition}
% %\label{definition4}
% \begin{definition}
% \label{definition3}
% Relative PC of $\hat{x}_{j,d}$ to $\hat{x}_{i,d}$ is defined by ${\rho}_{j/i,d} %(\bar{x}_{j,d}| \bar{x}_{i,d}) 
% = {\rho}_{j,d} / {\rho}_{i,d}=\alpha^{S_{j,d}-S_{i,d}}$.
% \end{definition}

% %By Definition 4, we can rewrite ${\rho}_{j/i,d}=\alpha^{S_{j,d}-S_{i,d}}$. Then, 
% According to Corollary \ref{corollary1}, the following corollary also holds.


% \begin{corollary}
% \label{corollary2}
% If $S_{i,d}=m\geq1$, then $\rho_{j/i,d} \in \{\alpha^{-1}, 1, \alpha\}\,$ for $v_j \in \mathcal{N}(v_i)$. Otherwise, if $S_{i,d}=0$, then $\rho_{j/i,d} \in \{ 1, \alpha\}\,$ for $v_j \in \mathcal{N}(v_i)$.
% \end{corollary}

% Corollary \ref{corollary2} shows that at the point of view of a missing node, there are only three possible cases for relative PC in its neighboring feature to its feature, while two cases for a source node.

Before defining a transition matrix, we reorder nodes temporarily according to whether a feature value is known or not for the $d$-th channel, i.e., $x^{(d)}$ and $A^{(d)}$ are reordered for each channel as described in \rv{Section~\ref{sub:notations}}. After the feature diffusion stage, we order the nodes according to the original numbering.

% Let $\tilde{X}=[\tilde{x}_{i,d}]$ denote an estimate of full feature $X$, which is updated via propagation steps in PC-based feature diffusion.
Built on \rv{Proposition \ref{proposition1}}, we construct a weighted adjacency matrix $W^{(d)}$ for the $d$-th channel. $W^{(d)} \in \mathbb{R}^{N \times N}$ is defined as follows,
\begin{equation}
    W^{(d)}_{i,j} = \begin{cases} \rho_{j/i,d} & \,\text{if} \; i \neq j \, , \, A^{(d)}_{i,j} = 1
    \\
    0 & \,\text{if} \; i \neq j \, , \, A^{(d)}_{i,j} = 0
    \\
    1 & \,\text{if} \; i = j\rv{.}
    \end{cases}
\end{equation}
Note that self-loops are added to $W^{(d)}$ with weight 1 so that each node can keep some of its own feature.

$W^{d}_{i,j}$ is an edge weight corresponding to message passing from $v_j$ to $v_i$. According to \rv{Proposition \ref{proposition1}}, $W^{(d)}_{i,j} \in \{\alpha^{-1}, 0, \alpha\}$ when $v_i$ and $v_j$ are connected. Hence, if we consider aggregation in a node, $\alpha^{-1}$ is assigned as edge weights for high-PC neighbors while 1 for same-PC and $\alpha$ for low-PC neighbors. That is, from a node's point of view, $W^{(d)}$ allows the node to aggregate more features with high PC from its neighbors. Furthermore, consider message passing between two connected nodes $v_i$ and $v_j$ s.t.  $\rho_{j/i,d}=\alpha$. By Definition~\ref{definition3}, $\rho_{i/j,d} = \rho^{-1}_{j/i,d}$, so that $W^{(d)}_{j,i} = (W^{(d)}_{i,j})^{-1} = \alpha^{-1}$. This means that message passing from a more confident node to a less confident node occurs with a large weight while message passing in the opposite direction occurs with a small weight.

To ensure convergence of diffusion process, we normalize $W^{(d)}$ to $\overline{W}^{(d)} =(D^{(d)})^{-1} W^{(d)}$ through row-stochastic normalization with $D^{(d)}_{ii} = \sum_j W_{i,j}$.
Since $x^{d}_k$ with true feature values should be preserved, we replace first $|\mathcal{V}^{(d)}|$ rows of $\overline{W}^{(d)}$ with one-hot vectors indicating $\mathcal{V}^{(d)}_k$. Finally, the channel-wise graph diffusion matrix $\widetilde{W}^{(d)}$
%a transition matrix 
for the $d$-th channel is expressed as
\begin{equation}
    \widetilde{W}^{(d)} = \begin{bmatrix}
I & \mathbf{0}_{ku} \\
\overline{W}^{(d)}_{uk} & \overline{W}^{(d)}_{uu}
\end{bmatrix} \rv{,}
\end{equation}
where $I\in \mathbb{R}^{|\mathcal{V}^{(d)}_k| \times |\mathcal{V}^{(d)}_k|} $ is an identity matrix and $\mathbf{0}_{ku} \in \{0\}^{|\mathcal{V}^{(d)}_k| \times |\mathcal{V}^{(d)}_u|}$ is a zero matrix. Note that $\widetilde{W}^{(d)}$ is still row-stochastic despite of the replacement.
An aggregation in a specific node can be regarded as a weighted sum of features on neighboring nodes. A row-stochastic matrix for transition matrix means that when a node aggregates features from its neighbors, the sum of the weights is 1. Therefore, unlike symmetric transition matrix~\cite{kipf2016semi, klicpera2019diffusion, rossi2021unreasonable} or column-stochastic (random walk) transition matrix~\cite{page1999pagerank, chung2007heat, perozzi2014deepwalk, grover2016node2vec, atwood2016diffusion, klicpera2018predict, lim2021class}, features of missing nodes can be formed at the same scale of known features. By preserving the original scale, features can be recovered close to the actual features.
% Since initial values usually have their own meaning unlike most features in neural networks, preserving the scale of initial feature can be extended to accurate simple feature prediction.

Now, we define channel-wise graph diffusion  for the $d$-th channel as
\begin{equation}
\begin{split}
&\tilde{x}^{(d)}(0) = \begin{bmatrix}
x^{(d)}_k\\
\mathbf{0}_u
\end{bmatrix}\\
   &\tilde{x}^{(d)} (t) = \widetilde{W}^{(d)} \tilde{x}^{(d)} (t-1)\rv{,}
\end{split}
\end{equation}
where $\tilde{x}^{(d)} (t)$ is a recovered feature for ${x}^{(d)}$ after $t$ propagation steps, $\mathbf{0}_u$ is a zero column vector of size $|\mathcal{V}^{(d)}_u|$ and $t \in [1,K]$. Note that we initialize missing feature values $x^{(d)}_u$ to zero. As $K \rightarrow \infty$, this recursion converges (the proof is included in the supplementary material). We approximate the steady state to $\tilde{x}^{(d)} (K)$, which is calculated by $(\widetilde{W}^{(d)})^K \tilde{x}^{(d)}(0)$ with large enough $K$. The diffusion is performed for each channel and outputs $\{\tilde{x}^{(d)}(K)\}^F_{d=1}$.

Because of the reordering nodes for each channel before the diffusion, node indices in $\tilde{x}^{(d)}(K)$ for $d\in \{1, ..., F\}$ are different. Therefore, after unifying different ordering in each $\tilde{x}^{(d)}(K)$ according to the original order in $X$, we concatenate all $\tilde{x}^{(d)}(K)$ along the channels into $\tilde{X}$ which is a final output in this stage.

\vspace{-0.2mm}

==> Neurips_2022/3.5-2.tex <==
 \subsection{Node-wise Inter-channel Propagation}
 \vspace{-0.3mm}
 \label{sub:ccp}
In the previous stage, we obtain $\tilde{X}=[\tilde{x}_{i,d}]$ (pre-recovered features for $X$) via channel-wise graph diffusion performed for each channel separately. The proposed feature diffusion is done based on the graph structure and pseudo-confidence, but does not consider dependency between channels. Since the dependency between channels can be another important factor for recovering missing node features, we develop an additional scheme to update $\tilde{X}$ by considering both channel correlation and pseudo-confidence.

We first prepare a covariance matrix $C = [C_{a,b}]\in \mathbb{R}^{F \times F}$ giving the covariance between each pair of channels for the proposed scheme. $C_{a,b}$, the covariance between $\tilde{X}_{:,a}$ and $\tilde{X}_{:,b}$ is calculated as
\begin{equation}
    C_{a,b} = \frac{1}{N-1} \sum^N_{i=1} (\tilde{x}_{i,a} - m_a )(\tilde{x}_{i,b} - m_b)\rv{,}
\end{equation}
where $m_d$ denotes the mean of a graph signal for the $d$-th channel, i.e., $m_d=\frac{1}{N}\sum^N_{i=1} \tilde{x}_{i,d}$.

In this stage, unlike looking across the nodes for each channel in the previous stage, we look across the channels for each node. As shown in the right-hand graph of Figure~\ref{fig:framework}, we define directed graphs $\{\mathcal{H}^{(i)}\}^N_{i=1}$ called node-wise inter-channel propagation graphs from the given graph $\mathcal{G}$. $\mathcal{H}^{(i)}$ for the $i$-th node in $\mathcal{G}$ is defined as
\begin{equation}
\mathcal{H}^{(i)} = (\mathcal{V}^{(i)}, \mathcal{E}^{(i)}, B^{(i)}) \rv{,}
\end{equation}
where $\mathcal{V}^{(i)}=\{v^{(i)}_d\}^F_{d=1}$ is a set of nodes in $\mathcal{H}^{(i)}$, $\mathcal{E}^{(i)}$ is a set of directed edges in $\mathcal{H}^{(i)}$, and $B^{(i)} \in \mathbb{R}^{F \times F}$ is a weighted adjacency matrix to update $\tilde{X}_{i,:}$. To update $\tilde{x}_{i,d}$ of the $i$-th node via inter-channel propagation, we assign $\tilde{x}_{i,d}$ to each $v^{(i)}_d$ as a \rv{scalar} node feature for the $d$-th channel ($d\in\{ 1, ..., F\}$). The weights in $\mathcal{E}^{(i)}$ are given by $B^{(i)}$, which will be described.

Our design goals of $B^{(i)}$ for inter-channel propagation in each node are to achieve threefold: (1) highly correlated channels should exchange more information to each other than less correlated channels, (2) a high PC channel feature should propagate more information to other channels of the node than a low PC channel feature, and (3) a low PC channel feature should receive more information from other channels for recovery than a high PC channel feature.
Based on these three design goals, 
the weight of the directed edge from the $b$-th channel to the $a$-th channel ($B^{(i)}_{a,b}$) in $B^{(i)}$ 
is designed by  
%we define $B^{(i)}$ as follows
\begin{equation}
\label{eq:matrixB}
B^{(i)}_{a,b} = \begin{cases} \gamma  (1-\alpha'^{S_{i, a}}) \frac{\alpha^{S_{i, b}}}{\sum^F_{b' \neq a}
\alpha^{S_{i, b'}}} %\sum^F_{b \neq a}
 C_{a,b}& \;\text{if} \; a \neq b 
    
    \\
    0 & \;\text{if} \; a = b
    \end{cases} \rv{,}
\end{equation}
where $C_{a,b}$, $\frac{\alpha^{S_{i, b}}}{\sum^F_{b' \neq a}
\alpha^{S_{i, b'}}}$, and $(1-\alpha'^{S_{i, a}})$ are terms to meet the design goal (1), (2), and (3), respectively.
$\alpha, \alpha' $ are hyperparameters for pseudo-confidence in Definition \ref{definition2}, and $\gamma$ is the scaling hyperparameter. Note that
we normalize the confidence, $\alpha^{S_{i, b}}$, to prevent too much increasing of aggregated channel features as $F$ increases. 
%Note that since the degree of aggregated channel features increases as $F$ increases, we normalize the edge weight by multiplying $\frac{1}{\sum^F_{b' \neq a}\alpha^{S_{i, b'}}}$.


%, and $m_b=\frac{1}{N}\sum^N_{i=1} \tilde{x}_{i,b}$.
% The self-loop weight $B_{d,d}^{(i)}$ derives each $v^{(i)}_d$ to preserve pre-recovered features $\tilde{x}_{i,d}$, while the other edge weights contribute to channel feature updates. %Note that $B^{(i)}_{a,b}$ is a weight of a directed edge corresponding to message passing to $v^{(i)}_a$ from $v^{(i)}_b$.

Node-wise inter-channel propagation on $\mathcal{H}^{(i)}$ outputs the final recovered features for $X_{i,:}$. We define node-wise inter-channel propagation as
\begin{equation}
\label{eq:Xhat}
\hat{X}^\top_{i,:} = \tilde{X}^\top_{i,:}+B^{(i)}(\tilde{X}_{i,:}-[m_1, \,m_2, \cdots,m_F])^\top \rv{,}
\end{equation}
where $\hat{X}_{i,:}$ and $\tilde{X}_{i,:}$ are row vectors.
Preserving the pre-recovered channel feature values (as self loops), message passing among different channel features is done along the directed edges of $B^{(i)}$. After calculating $\hat{X}_{i,:}$ for $i \in \{1, ...,N\}$, we obtain the final recovered features by concatenating them, i.e., $\hat{X} = [{\hat{X}_{1, :}}^\top\; {\hat{X}_{2, :}}^\top \;\, \cdots \;\, {\hat{X}_{N, :}}^\top]^\top$. Moreover, since $C$ is calculated via pre-recovered features $\tilde{X}$ for all nodes in $\mathcal{G}$, channel correlation propagation injects global information into recovered features for $X$. $\hat{X}$ is a final output of PC-based feature recovery and is fed to GNN to solve a downstream task.
\vspace{-0.6mm}

% Preserving the pre-recovered feature values, message passing is done using deviation of each channel feature along the directed edges. Hence $i$-th row vector of $\hat{X}$, i.e.$\hat{X}_{i,:}$ becomes
% \begin{equation}
% \label{eq:Xhat}
% \hat{X}_{i,:} = \tilde{X}^\top_{i,:}+B^{(i)}(\tilde{X}_{i,:}-[m_1, \,m_2, \cdots,m_F])^\top,
% \end{equation}
% where $\hat{X}_{i,:}$ and $\tilde{X}_{i,:}$ are row vectors. After calculating $\hat{X}_{i,:}$ for $i \in \{1, ...,N\}$, we obtain the final recovered features by concatenating them, i.e., $\hat{X} = [{\hat{X}_{1, :}}^\top\; {\hat{X}_{2, :}}^\top \;\, \cdots \;\, {\hat{X}_{N, :}}^\top]^\top$. Moreover, since $C$ is calculated via pre-recovered features $\tilde{X}$ for all nodes in $\mathcal{G}$, channel correlation propagation injects global information into recovered features for $X$. $\hat{X}$ is a final output of PC-based feature recovery (PCFR) and is fed to GNN to solve a downstream task.

==> Neurips_2022/4-Experiments_0.tex <==
\section{Experiments}
\label{Experiments}
\vspace{-0.3mm}
\input{4.1-0}
% \input{4.2-0}
\input{4.3-1}
\input{4.4-1}
\input{4.5-1}

==> Neurips_2022/4.1-0.tex <==
\subsection{Datasets}
\label{sub:datasets}
\vspace{-0.4mm}
% 실험 결과를 작성할 페이지가 많이 부족할 것 같아서 간략히 작성하고 실험에 대한 자세한 설명은 appendix에 작성하려고 했습니다. 만약 자세한 작성이 필요하다면, 추가하도록 하겠습니다.
To validate our method, we conducted experiments on 6 benchmark datasets from two different domains: Citation networks (Cora, CiteSeer, PubMed~\cite{sen2008collective}, and OGBN-Arxiv~\cite{hu2020open}) and Recommendation networks (Amazon-Computers and Amazon-Photo~\cite{shchur2018pitfalls}). \rv{For link prediction, we evaluated methods on the 5 benchmark datasets except OGBN-Arxiv which causes out of memory.} The description for the datasets are reported in the supplementary material.


==> Neurips_2022/4.2-0.tex <==
\subsection{Baselines}
\label{sub:baselines}

We compared our method with two baselines and four state-of-the-art methods. we set baseline 1 as a simple way to utilize a GNN for graph with missing feature. All missing values in a feature matrix are set to zero and the features are fed to a GNN in Baseline 1. We set Baseline 2 as label propagation (LP)~\cite{zhu2002learning} which can be a solution for 100\% feature missing, since LP infers labels by simply diffusing given labels. The four compared state-of-the-art methods can be categorized into two approaches: \textit{GCN-variant model}=\{GCNMF~\cite{taguchi2021graph}, PaGNN~\cite{jiang2020incomplete}\} and \textit{feature imputation}= \{sRMGCNN~\cite{monti2017geometric}, FP~\cite{rossi2021unreasonable}\}. For baseline 1, sRMGCNN, FP, and our method, GCN is adopted as a downstream GNN. For all the methods based on GCN, the number of layers is set to 3.

==> Neurips_2022/4.3-0.tex <==
\subsection{Experimental Setup}
\label{sub:experimentalsetup}
\vspace{-0.3mm}
{\bf Compared Methods.} We compared our method with two baselines and four state-of-the-art methods. we set {\bf Baseline 1} to a simple scheme that directly feeds the graph data with missing features to  GNN without recovery, where %baseline 1 as a simple way to utilize a GNN for graph with missing feature. 
all missing values in a feature matrix are set to zero.
%and the features are fed to  Baseline 1.
We set {\bf Baseline 2} to label propagation (LP)~\cite{zhu2002learning} which does not use node features and propagates only partially-known labels for inferring the remaining labels. That is, LP corresponds to the case of 100\% feature missing.
%can be a solution for 100\% feature missing, since LP infers labels by simply diffusing given labels, i.e., LP does not use any feature. 
The four  state-of-the-art methods can be categorized into two approaches: \textit{GCN-variant model}=\{GCNMF~\cite{taguchi2021graph}, PaGNN~\cite{jiang2020incomplete}\} and \textit{feature imputation}= \{sRMGCNN~\cite{monti2017geometric}, FP~\cite{rossi2021unreasonable}\}. For Baseline 1, sRMGCNN, FP, and our method,  vanilla GCN~\cite{kipf2016semi} is used only for the downstream task.
%GCN is adopted as a downstream GNN. 
For GCN-variant  models perform both feature recovery and downstream task in the GCN framework where a scheme for feature recovery is added to vanilla GCN.
In all the compared methods, the same GCN ~\cite{kipf2016semi} is used.
%based on GCN, the number of layers is set to 3.
\vspace{-0.3mm}

{\bf Data Settings.} We randomly generated 10 different training/validation/test splits for semi-supervised node classification,  except OGBN-Arxiv where the split was fixed according to the specified criteria. In each generated split, 20 per class were assigned to  the training set and a total of 1500 nodes were assigned to the validation set regardless of class.
%1500 in total, respectively. 
For the test set, we used all nodes except training and validation nodes. We removed features according to missing rate $r_m$ ($0< r_m<1$). Missing features were selected in two ways as follows.
%the following two ways:
\vspace{-0.6mm}
\begin{itemize}
    \item \textbf{\textit{Structural missing}.} We first randomly selected nodes in a ratio of $r_m$ among all nodes. Then, we assigned all features of the selected nodes to missing (unknown) values (zero).
    \vspace{-0.3mm}
    \item \textbf{\textit{Uniform missing}.} We randomly selected features in a ratio of $r_m$ from the node feature matrix $X$, and we set the selected features to missing (unknown) values (zero).
\end{itemize}
\vspace{-0.6mm}

{\bf Evaluation.} For each missing type, we report the node classification accuracy evaluated on 10 different pairs of splits for node labels and missing features.
To ensure a fair comparison, we employed the same standard hyperparameters for training across all methods. A detailed description of the hyperparameters used in experiments and implementation of each method are given in the supplementary material.



==> Neurips_2022/4.3-1.tex <==
\subsection{Experimental Setup}
\label{sub:experimentalsetup}
\vspace{-0.3mm}
{\bf Compared Methods.} For semi-supervised node classification, we compared our method with two baselines and four state-of-the-art methods. we set {\bf Baseline 1} to a simple scheme that directly feeds the graph data with missing features to  GNN without recovery, where %baseline 1 as a simple way to utilize a GNN for graph with missing feature. 
all missing values in a feature matrix are set to zero.
%and the features are fed to  Baseline 1.
We set {\bf Baseline 2} to label propagation (LP)~\cite{zhu2002learning} which does not use node features and propagates only partially-known labels for inferring the remaining labels. That is, LP corresponds to the case of 100\% feature missing.
%can be a solution for 100\% feature missing, since LP infers labels by simply diffusing given labels, i.e., LP does not use any feature. 
The four  state-of-the-art methods can be categorized into two approaches: \textit{GCN-variant model}=\{GCNMF~\cite{taguchi2021graph}, PaGNN~\cite{jiang2020incomplete}\} and \textit{feature imputation}= \{sRMGCNN~\cite{monti2017geometric}, FP~\cite{rossi2021unreasonable}\}. For Baseline 1, sRMGCNN, FP, and our method,  vanilla GCN~\cite{kipf2016semi} is used only for the downstream task.
%GCN is adopted as a downstream GNN. 
For GCN-variant models perform both feature recovery and downstream task in the GCN framework where a scheme for feature recovery is added to vanilla GCN.
In all the compared methods, the same GCN ~\cite{kipf2016semi} is used.
%based on GCN, the number of layers is set to 3.

\rv{For link prediction, we compared our method with sRMGCNN and FP, which are the feature imputation approach. To perform link prediction on the inferred features by each method, graph auto-encoder (GAE)~\cite{kipf2016variational} models are adopted. We used inferred features by each method as input of GAE models.}

\vspace{-0.2mm}

{\bf Data Settings.}  \rv{Regardless of the type of task, we} removed features according to missing rate $r_m$ ($0< r_m<1$). Missing features were selected in two ways as follows.
%the following two ways:
\vspace{-0.3mm}
\begin{itemize}
    \item \textbf{\textit{Structural missing}.} We first randomly selected nodes in a ratio of $r_m$ among all nodes. Then, we assigned all features of the selected nodes to missing (unknown) values (zero).
    \vspace{-0.3mm}
    \item \textbf{\textit{Uniform missing}.} We randomly selected features in a ratio of $r_m$ from the node feature matrix $X$, and we set the selected features to missing (unknown) values (zero).
\end{itemize}

For semi-supervised node classification, we randomly generated 10 different training/validation/test splits, except OGBN-Arxiv where the split was fixed according to the specified criteria. In each generated split, 20 per class were assigned to  the training set and a total of 1500 nodes were assigned to the validation set regardless of class. For the test set, we used all nodes except training and validation nodes.

\rv{For link prediction, we also randomly generated 10 different training/validation/test splits for each datasets. We split edges with the same split ratio for all the datasets. As in the setting in ~\cite{kipf2016variational}, we used 85\% edges for train, 5\% edges for validation, and the 10\% edges for test.}

\vspace{-0.3mm}

\input{figure-comparison}

\input{tables/sota_table}

{\bf Evaluation.} \rv{For node classification, we report the accuracy evaluated on 10 different pairs of splits for node labels and missing features. For link prediction, we report area under the ROC curve (AUC) and average precision (AP) scores on 10 different pairs of splits for edges and missing features.} A detailed description of the hyperparameters used in experiments and implementation of each method are given in the supplementary material.

\clearpage

==> Neurips_2022/4.4-0.tex <==
\subsection{Resistance of PCFR to missing features}
\label{sub:resistance}

% \input{tables/resistance_table}
\vspace{-0.3mm}
To verify the resistance of PCFR against missing features, we compared the averaged node classification accuracy for the 6 datasets by increasing $r_m$. We compared each average accuracy with different $r_m$ from $r_m=0$ to $r_m=0.95$. For structural missing, PCFR loses only 2.24\% of relative average accuracy with $r_m = 0.9$, and 4.86\% with $r_m = 0.995$. In the case of uniform missing, PCFR loses only 1.61\% of relative average accuracy with $r_m = 0.9$, and 2.99\% with $r_m = 0.995$. Note that classification with $r_m=0.995$ is the extremely missing case in which only 0.5\% of features are known. This result demonstrates that PCFR is \rv{robust} to missing features.
\vspace{-0.3mm}

Even at the same $r_m$, we observed the average accuracy for structural missing is lower than one for uniform missing. We analyzed this observation in the aspect of confidence. Since features are missing in a node unit for structural missing, all channel features of a node have the same SPD-S, i.e., $S_{i,1}=\ldots = S_{i,F}$. Hence, in a node far from its nearest source node, every channel feature has low confidence. Then, every missing feature of the node can not be improved via node-wise inter-channel propagation due to absence of highly confident channel features in the node. Thus, the node is likely to be misclassified. In contrast, for uniform missing, channel features of a node have various PC where known channel features have high confidence and propagate their feature information to unknown channel features in the node. Hence, most nodes can be classified well owing to the recovered features from highly confident channel features. We claim that this observation shows the validity of the concept of channel-wise confidence. The table containing accuracy at different $r_m$ for the two missing types is in the supplementary material.
\vspace{-0.1mm}
\input{figure-comparison}

\input{tables/sota_table}

==> Neurips_2022/4.4-1.tex <==
\rv{\subsection{Semi-Supervised Node Classification Results}}
\vspace{-0.2mm}
\label{sub:ncr}



Figure~\ref{fig:comparison} 
demonstrates the trend of  average accuracy of compared methods for node classification on 6 datasets with different $r_m$. The performance gain of PCFR is remarkable at $r_m = 0.995$. In contrast, the average accuracy of existing methods rapidly decrease as $r_m$ increases and are overtaken by LP which does not utilize features. In the case of uniform missing features, FP shows better resistance than LP, but the gap from ours increases as $r_m$ increases.
%While LP shows the highest performance for OGBN-Arxiv with $r_m = 99.5\%$, the performance of LP for a dataset is constant regardless of $r_m$, i.e., LP shows low performance in all cases except extremely high $r_m$. Moreover, since LP is designed only for node classification and can not be applied to other downstream tasks. 
The high performance of PCFR comes from the proposed channel-wise confidence which is an important concept to deal with missing channel features. \rv{We conclude that PCFR effectively contributes to performance improvement of node classification.}



Table~\ref{sota_table} shows the detailed results of node classification with $r_m=0.995$. 
sRMGCNN and GCNMF show significantly low performance for all experiments in this extremely challenging environment. \rv{Even PaGNN shows worse accuracy than Baseline 2 (LP) in general.}
%Most existing methods suffer large performance degradation at a high rate of missing features, which leads to performance comparable to or lower than LP except for FP in the uniform missing case with $r_m = 0.995$. 
For all the datasets except OGBN-Arxiv, PCFR shows superior performance to the other methods at $r_m = 0.995$.
Ablation study to analyze the effectiveness of channel-wise graph diffusion and node-wise inter-channel propagation is provided in the supplementary material.



==> Neurips_2022/4.5-0.tex <==
\subsection{Comparison with State-of-the-art Methods}
\vspace{-0.2mm}
\label{sub:comparison}





%Table~\ref{sota_table} shows the results of node classification with $r_m=99.5\%$. sRMGCNN and GCNMF show significantly low performance for all experiments at $r_m = 99.5\%$. Even PaGNN and FP outperform LP only in some experiments. The existing methods suffer large performance degradation at a high rate of missing features, which leads to performance comparable to or lower than LP except for FP in the uniform missing case with $r_m = 0.995$. For all the datasets except OGBN-Arxiv, PCFR shows superior performance to the other methods at $r_m = 99.5\%$.

Figure~\ref{fig:comparison} demonstrates the trend of  average accuracy of compared methods for node classification on 6 datasets with different $r_m$. The performance gain of PCFR is remarkable at $r_m = 0.995$. In contrast, the average accuracy of existing methods rapidly decrease as $r_m$ increases and are overtaken by LP which does not utilize features. In the case of uniform missing features, FP shows better resistance than LP, but the gap from ours increases as $r_m$ increases.
%While LP shows the highest performance for OGBN-Arxiv with $r_m = 99.5\%$, the performance of LP for a dataset is constant regardless of $r_m$, i.e., LP shows low performance in all cases except extremely high $r_m$. Moreover, since LP is designed only for node classification and can not be applied to other downstream tasks. 
The high performance of PCFR comes from the proposed channel-wise confidence which is an important concept to deal with missing channel features. We conclude that PCFR effectively recovers missing features for the downstream task.

Table~\ref{sota_table} shows the detailed results of node classification with $r_m=0.995$. 
sRMGCNN and GCNMF show significantly low performance for all experiments in this extremely challenging environment. Even PaGNN and FP show worse accuracy than Baseline 2 (LP) except  some datasets. 
%Most existing methods suffer large performance degradation at a high rate of missing features, which leads to performance comparable to or lower than LP except for FP in the uniform missing case with $r_m = 0.995$. 
For all the datasets except OGBN-Arxiv, PCFR shows superior performance to the other methods at $r_m = 0.995$.


==> Neurips_2022/4.5-1.tex <==
\rv{\subsection{Link Prediction Results}}
\vspace{-0.2mm}
\label{sub:ncr}

\input{tables/link_pre_table}

\rv{Table~\ref{tab:lp} demonstrates results for the link prediction task at $r_m$=0.995. While GCNMF, PaGNN can only deal with node classification, feature imputation methods can be applied to link prediction. Among them, PCFR achieves state-of-the-art
performance across all the datasets. Based on the results on semi-supervised node classification and link prediction, which are representative graph learning tasks, PCFR shows the effectiveness at a very high rate of missing features.}

Ablation study to analyze the effectiveness of channel-wise graph diffusion and node-wise inter-channel propagation is provided in the supplementary material.

==> Neurips_2022/5-Conclusion_0.tex <==

\section{Conclusion}
\label{Conclusion}
\vspace{-0.4mm}
We introduced a novel concept of channel-wise confidence to recover highly-rated missing features in a graph. To replace the unavailable true confidence, we designed a pseudo-confidence that can be obtained from the shortest path distance of each channel feature of a node. Using the pseudo-confidence, we developed a new framework for missing feature recovery that consists of channel-wise graph diffusion and node-wise inter-channel propagation.
%, an essential factor for handling graphs with missing features. 
%Confidence assigned to each recovered feature value represents a degree of confidence in the recovered value. 
%We have further proposed PCFR to solve a missing feature recovery problem by considering confidence. 
As validated in experiments, the proposed method shows outperforming performance \rv{on both node classification and link prediction}. The channel-wise confidence approach for missing feature recovery can be easily applied to various graph-related downstream tasks with missing node features.
%Extensive experimental results demonstrate the validity of confidence and the effectiveness of PCFR that achieves state-of-the-art performance.
%Moreover, PCFR can be applied to not only node classification but also various graph-related tasks with missing node features. Since feature missing in networks is common in real-world scenarios, confidence is expected to be one of the bases for graph learning applications.

% \textbf{Limitation.} As most GNNs consider graphs with high homophily, our method is also designed under homophily assumption (connected nodes are similar). %Thus, future work should be designed for missing feature recovery on graphs with low homophily.
% However, many real-world networks are not limited to pairwise relations or high homophily structure.
% Therefore, it is an interesting future work to extend our work to more challenging structures such as hypergraphs modeling higher-order relations or highly heterophily graphs whose connected nodes are opposite each other.
\vspace{-0.2mm}
\textbf{Limitation.} Many real-world networks are not limited to pairwise relations or single-type nodes adopted in our work. Therefore, it is an interesting future work to extend our work to more challenging structures such as hypergraphs for modeling higher-order relations or heterogeneous graphs with multi-type nodes.

\vspace{-0.2mm}
\textbf{Potential negative societal impacts.}
%Our work aims to recover missing features from known features on graphs. The work can be applied to real-world networks such as social networks and web pages. However, 
The intentionally removed private or confidential information can be recovered by using the proposed method and the recovered information can be misused.  
%side effects can occur when inferred features containing private information or company confidential information are misused. 
Therefore, the work is suggested to be used with an aim for positive impacts on society such as health care~\cite{wang2020guardhealth, deng2020cola}, crime prediction~\cite{wang2021hagen}, and weather forecasting~\cite{han2022semi}.

==> Neurips_2022/figure-acc-citeseer.tex <==
\begin{figure*}[h!]
\begin{center}
\includegraphics[width = 0.8\linewidth]{figures/acc_con.PNG}
\end{center}
\vspace{-0.7mm}
\rv{
\caption{Node classification accuracy (\%) according to SPD-S of test nodes. For both Cora and CiteSeer, structural missing with $r_m = 0.995$ is applied. PCFR* denotes PCFR without node-wise inter-channel propagation.}}
\label{fig:acc}
\vspace{-2.5mm}
\end{figure*}

==> Neurips_2022/figure-comparison.tex <==
\begin{figure*}[t]
\centerline{\includegraphics[width=0.8\linewidth]{figures/comparison_dh.pdf}}
\vspace{-2.8mm}
\caption{Average accuracy (\%) on the 6 datasets with $r_m \in \{0, 0.5, 0.9, 0.995\}$. sRMGCNN and GCNMF are excepted due to OOM results in some datasets and the significantly poor performance on all the available datasets as shown in table~\ref{sota_table}.}
\label{fig:comparison}
\end{figure*}


==> Neurips_2022/figure-framework.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width = 0.99\linewidth]{figures/framework_final_2.PNG}
\end{center}
\vspace{-0.7mm}
\caption{Overall scheme of the proposed Pseudo-Confidence based Feature Recovery (PCFR) method. Based on the graph structure and partially known features, we calculate the channel-wise shortest path distance between a node with a missing feature and its nearest source node (SPD-S). Based on SPD-S, we determine the pseudo-confidence in the recovered feature, using a pre-determined hyperparameter $\alpha \,(0<\alpha<1)$. Pseudo-confidence plays an important role in our two stages: channel-wise graph diffusion and node-wise inter-channel propagation.}
\label{fig:framework}
\vspace{-2.5mm}
\end{figure*}

==> Neurips_2022/figure-gamma.tex <==
\begin{figure*}[h!]
\begin{center}
\includegraphics[width = 0.99\linewidth]{figures/gamma.PNG}
\end{center}
\caption{Accuracy with different $\gamma$ under a structural-missing setting with $r_m = 0.995$. For Cora and CiteSeer, $(\alpha, \alpha')$ is set to $(0.8, 0.4)$ and $(0.8, 0.3)$, respectively. Each horizontal green line denotes the accuracy with $\gamma=0$, which represents performance of PCFR without node-wise inter-channel propagation. \rv{The shaded area denotes the standard deviation of classification accuracy.}}
\label{fig:gamma}
\end{figure*}

==> Neurips_2022/figure-heatmap.tex <==
\begin{figure*}[h!]
\begin{center}
\includegraphics[width = 0.99\linewidth]{figures/heatmap4.PNG}
\end{center}
\caption{Accuracy on Cora and CiteSeer with different $\alpha$ and $\alpha'$. The experiments on each dataset are conducted under a structural-missing setting with $r_m = 0.995$ and $\gamma=10^3$.}
\label{fig:heatmap}
\end{figure*}

==> Neurips_2022/figure-sim-citeseer.tex <==
\begin{figure*}[h!]
\begin{center}
\includegraphics[width = 0.8\linewidth]{figures/sim_con.PNG}
\end{center}
\vspace{-0.7mm}
\caption{\rv{Cosine similarity between original features and recovered features according to SPD-S of overall nodes. For both Cora and CiteSeer, structural missing with $r_m = 0.995$ is applied. PCFR* denotes PCFR without node-wise inter-channel propagation.}}
\label{fig:sim}
\vspace{-2.5mm}
\end{figure*}

==> Neurips_2022/figure-time.tex <==
\begin{figure*}[h!]
\begin{center}
\includegraphics[width = 0.65\linewidth]{figures/time3.PNG}
\end{center}
\caption{Training time (in seconds) of methods on Cora under a structural-missing setting with $r_m = 0.995$.}
\label{fig:time}
\end{figure*}

==> Neurips_2022/figure_dim_structural.tex <==
\begin{figure*}[h!]
\begin{center}
\includegraphics[width = 0.95\linewidth]{figures/dim_structural.PNG}
\end{center}
\caption{Node classification accuracy (\%) under a structural missing setting with $r_m=0.995$. The hidden dimension is increased from 16 to 128 by multiplying 2 while fixing the number of layers to 3.}
\label{fig:gamma}
\end{figure*}

==> Neurips_2022/figure_dim_uniform.tex <==
\begin{figure*}[h!]
\begin{center}
\includegraphics[width = 0.95\linewidth]{figures/dim_uniform.PNG}
\end{center}
\caption{Node classification accuracy (\%) under a uniform missing setting with $r_m=0.995$. The hidden dimension is increased from 16 to 128 by multiplying 2 while fixing the number of layers to 3.}
\label{fig:gamma}
\end{figure*}

==> Neurips_2022/figure_layer_structural.tex <==
\begin{figure*}[h!]
\begin{center}
\includegraphics[width = 0.95\linewidth]{figures/layer_structural.PNG}
\end{center}
\caption{Node classification accuracy (\%) under a structural missing setting with $r_m=0.995$. The number of layers is increased from 2 to 4 while fixing the hidden dimension to 64.}
\label{fig:gamma}
\end{figure*}

==> Neurips_2022/figure_layer_uniform.tex <==
\begin{figure*}[h!]
\begin{center}
\includegraphics[width = 0.95\linewidth]{figures/layer_uniform.PNG}
\end{center}
\caption{Node classification accuracy (\%) under a uniform missing setting with $r_m=0.995$. The number of layers is increased from 2 to 4 while fixing the hidden dimension to 64.}
\label{fig:gamma}
\end{figure*}

==> Neurips_2022/figure_performance.tex <==
\begin{figure*}[h!]
  \centering
  \includegraphics[clip,trim={0 5cm 0 0}, width=0.73\linewidth]{figures/perf_per_data.pdf}
  \caption{Average accuracy (\%) for each setting (missing type, dataset).}
\end{figure*}

==> previous_version/1-Intro_0.tex <==
\section{Introduction}

In recent years, graph neural networks (GNNs) have received a lot of attention and have shown outstanding performance on numerous problems in various fields~\cite{zhou2020graph, wu2020comprehensive, zhang2020deep,zitnik2018modeling,ying2018graph, chen2019multi, narasimhan2018out, yan2018spatial, yao2019graph, fout2017protein}. A key aspect of GNN is a message passing \cite{gilmer2017neural} which updates node representation by aggregating features of its neighbors and itself. Under the framework of the message passing schemes, GNNs learn node feature embedding from initial node features via leveraging graph structure.

GNN models typically assume that features for all nodes are fully observed. However, in real-world situations, features in graph-structured data are often partially observed as illustrated in the following cases. First, collecting complete data for a large graph is expensive or even impossible. Secondly, in social networks, most users want to protect their personal information selectively. Besides, measurement failure or newly joined nodes after measurement happens often. Most existing GNN models cannot be directly applied to the above situations.



%%% 기존 방식의 문제와 confidence 방식을 왜 써야하는지. 아래와 연결이 자연스롭도록 조금 수정하면 좋겠습니다.

To tackle this problem, several feature imputation methods~\cite{rossi2021unreasonable, chen2020learning} and extended-GNN methods~\cite{taguchi2021graph, jiang2020incomplete} have been proposed. Despite their reasonable performance at low rates of missing features, these methods cannot avoid significant performance degradation at a high rate of missing features. The underlying assumption across all methods as well as message passing methods via GNNs is $\textit{homophily}$ which represents the concept that linked nodes often belong to the same class and have similar features~\cite{mcpherson2001birds}. However, since homophily is a local property~\cite{bisgin2010investigating, lauw2010homophily, bisgin2012study}, inferring missing features from sparse known features by only relying on homophily probably leads to inaccurate results due to trivial feature passing.

% To tackle this problem,  feature imputation methods~\cite{rossi2021unreasonable, chen2020learning} and extended-GNN methods~\cite{taguchi2021graph, jiang2020incomplete} have been proposed.
% Despite their reasonable performance at low rates of missing features, these methods cannot avoid significant performance degradation at a high rate of missing features. 
% When features are missing at high rates ($ \geq 90\%$),  one node might have no neighbor node which has feature information and have to fill its missing features from distant nodes by message passing.
% In this case, naively treating the message from the distant node as the one from a directly linked node can lead to inaccurate feature learning.
% Also, the reliability of a message would be different between actual feature and the inferred feature.
% Therefore, messages need to be propagated differently according to its reliability.

% 위에서 (1-> 해결이 confidence 방식이고, 2->의 해결이 channel-wise, node-wise propagation.)로 자연스럽게 연결하면 좋을듯. 

% To this end, we define a new concept of {\it confidence} 
% which is assigned to a recovered feature for reflecting uncertainty of the recovery. 
% To replace unavailable true confidence in actual learning process, we suggest {\it pseudo-confidence} calculated by the shortest path distance between a missing-feature node and its nearest known-feature node for each channel. 

To overcome the aforementioned limitation, we define a new concept of {\it confidence} which is assigned to a recovered feature for reflecting uncertainty of the recovery. To replace unavailable true confidence in actual learning process, we suggest {\it pseudo-confidence} calculated by the shortest path distance between a missing-feature node and its nearest known-feature node for each channel. 
Using pseudo-confidence, we develop a pseudo-confidence based feature recovery (PCFR) scheme consisting of two stages: Channel-wise Between-node
Diffusion and Node-wise Between-channel Propagation for missing feature recovery from known features. 
Through extensive experiments on various datasets containing a very high rate of missing features, we validate the proposed PCFR is strongly resistant to missing features and shows state-of-the-art accuracy for node classification. 

The key contribution of our work can be summarized as follows: (1) We propose a new concept of confidence that represents the quality of a recovered feature based on similarity between a recovered feature and a true one.
(2) We design a method to give pseudo-confidence that can be replaced instead of unavailable true confidence. 
(3) Based on the pseudo-confidence, we propose a novel feature recovery scheme which achieves the state-of-the-art accuracy for node classification even in a very high missing rate (e.g. 99.5\%) of missing features.

% contribution
% (1) confidence라는 개념을 새롭게 제안
% (2) 기존의 Distance encoding과 다르다.
% (3) robust to a very high rate of missing features
% (4) 확장성

==> previous_version/1-Intro_1.tex <==
\section{Introduction}
\label{Intro}
In recent years, graph neural networks (GNNs) have received a lot of attention and have shown outstanding performance on numerous problems in various fields~\cite{zhou2020graph, wu2020comprehensive, zhang2020deep,zitnik2018modeling,ying2018graph, chen2019multi, narasimhan2018out, yan2018spatial, yao2019graph, fout2017protein}. GNN models typically assume that features for all nodes are fully observed. However, in real-world situations, features in graph-structured data are often partially observed as illustrated in the following cases. First, collecting complete data for a large graph is expensive or even impossible. Secondly, in social networks, most users want to protect their personal information selectively. Besides, measurement failure or newly joined nodes after measurement happens often. Under these situations, most GNNs cannot be directly applied due to incomplete features.

To tackle this problem, several methods are proposed by the following two approaches: structurally modified GNN~\cite{taguchi2021graph, jiang2020incomplete} and feature imputation~\cite{monti2017geometric, rossi2021unreasonable}. At a high rate of missing features, while structurally modified GNN approaches suffer significant performance degradation, feature propagation (FP)~\cite{rossi2021unreasonable} prevent large performance drop. FP recovers missing features by spreading known features to their neighboring nodes. However, we observe that as a rate of missing features increase, the performance of FP decreases and is eventually caught up with the performance of a method not using any feature~\cite{zhu2002learning}.

When we assume a graph with a high rate of missing features, there are two kinds of sparsity of known feature values: (1) sparsity across nodes for a specific channel and (2) sparsity in feature of a node. For (1), we consider aggregation at a missing feature value. In FP, a missing feature is recovered by aggregating features from connected nodes regardless of whether known feature or recovering feature. However, we cannot be completely confident in a recovered value while a known feature value is true value. Moreover, due to the $homophily$ (the phenomenon that linked nodes often belong to the same class and have similar features~\cite{mcpherson2001birds}), two nodes with a large shortest path distance between them are probably dissimilar. Thus, if we infer all node features in a graph as a single known feature, features of nodes close to the node with known feature may be more similar to their true value than the others. That is, there will be different degrees of certainty even between inferred features. For (2), we then consider pre-recovered feature of a node, which is obtained by spreading known features. Since pre-recovered values for missing values are not exactly accurate, using known feature values in the node may help recovery.

Motivated by these two considerations, we first define a novel concept of {\it confidence} that represents a degree of confidence in each feature value. Since it is not possible to obtain defined confidence for missing values, we suggest {\it pseudo-confidence} calculated using the graph structure. Built on pseudo-confidence, we develop a pseudo-confidence based feature recovery (PCFR) scheme consisting of two stages: Channel-wise Between-node Diffusion and Node-wise Between-channel Propagation for missing feature recovery from known features. Through extensive experiments on various datasets containing a very high rate of missing features, we validate the proposed PCFR is strongly resistant to missing features and shows state-of-the-art accuracy for node classification.

The key contribution of our work can be summarized as follows: (1) We propose a new concept of confidence that represents the quality of a recovered feature.
(2) We design a method to give pseudo-confidence that can be replaced instead of unavailable true confidence.
(3) Based on the pseudo-confidence, we propose a novel feature recovery scheme which achieves the state-of-the-art accuracy for node classification even in a very high missing rate (e.g. 99.5\%) of missing features.

==> previous_version/1-Intro_tmp.tex <==

\section{Introduction}

% 1문단: graph에서 missing 문제와 해결 방법
In recent years, graph neural networks (GNNs) have received a lot of attention and have shown outstanding performance on numerous problems in various fields~\cite{zhou2020graph, wu2020comprehensive, zhang2020deep,zitnik2018modeling,ying2018graph, chen2019multi, narasimhan2018out, yan2018spatial, yao2019graph, fout2017protein}. GNN models typically assume that features for all nodes are fully observed. However, in real-world situations, features in graph-structured data are often partially observed as illustrated in the following cases. First, collecting complete data for a large graph is expensive or even impossible. Secondly, in social networks, most users want to protect their personal information selectively. Besides, measurement failure or newly joined nodes after measurement happens often. Under these situations, most GNNs cannot be directly applied due to incomplete features.

% 2문단: extremely missing 높아질 때는 단순한 diffusion으로 잘 안됨. 그냥 단순히 같은 weight로 합치는 게 아니고 중요도 (confidence) 고려해주어야 함.  
Recently, several methods~\cite{monti2017geometric, jiang2020incomplete, taguchi2021graph, rossi2021unreasonable} have been proposed to handle missing features in graphs. 
However, these methods suffer from significant performance degradation at high missing feature rates ($\geq 99\%$).
In real-world scenarios, extremely sparse data~\cite{ref:wind_data, ref:extreme_sparse_18} commonly exist, which is significant but challenging.
While Feature Propagation (FP)~\cite{rossi2021unreasonable}, which recovers missing features by aggregating features from connected nodes, shows improved performance, it still cannot avoid a considerable accuracy drop when the missing rate increases up to $99.5\%$.
It is because when the missing rate is extremely high and the known features are sparsely distributed, some features cannot but be recovered from the features which are also inferred from distant nodes having the known features. 
However, the `confidence' in the information (message) differs between the actual (known) features and the features inferred through several nodes.
That is, the known features should have the highest importance when propagating the features to their neighboring nodes.
Hence, for robust reconstruction of unknown features, each feature needs to be diffused with different weights according to their importance to a missing feature.

% 3문단: 왜 confidence/pseudo-confidece 써야하는지 
From the above motivation, we raise the following questions:
\textit{How can we measure the importance of features? and how can we better diffuse features for robust reconstruction from a graph with extremely missing features?}
First, to measure the importance, we define a new concept of {\it confidence}, which measures how similar the recovered features are to the actual features.
That is, perfectly recovered features should have the highest importance for diffusion.
However, since {\it confidence} is not available in training process, we propose {\it pseudo-confidence}.
Based on the feature homophily assumption in GNNs (i.e., that linked nodes are likely to have similar features)~\cite{mcpherson2001birds, wang2021hagen, rossi2021unreasonable}, we assume that features between two distant nodes are likely to be dissimilar (i.e., low confidence).
From this intuition, {\it pseudo-confidence} is calculated by the shortest path distance between a missing-feature node and its nearest known-feature node. 

% 4문단: 왜 channel-wise between-node, node-wise between-channel 써야하는지?
Second, to better diffuse features, we propose channel-wise between-node diffusion and node-wise between-channel propagation based on pseudo-confidence, in contrast to the existing methods that simply use the entire features.
For example, assume a node represents a user and features represent items (e.g., preference for dog, cat, fish).
In this case, global statistics of a `dog' between all users can be utilized when inferring missing preference of a `dog' for one user (i.e., channel-wise between-node diffusion).
Also, we can utilize the statistics within each user to reflect different preferences (i.e., node-wise between-channel).
From this intuition, we propose different types of propagation for robust reconstruction of missing features.


% 결론.
Therefore, we propose a novel pseudo-confidence based feature recovery (PCFR) scheme consisting of two stages: Channel-wise Between-node Diffusion and Node-wise Between-channel Propagation for missing feature recovery from known features.
Through extensive experiments on various datasets with different levels of missing features, we demonstrate the validity of our method, and show that PCFR is robust to extremely high rates of missing features.
Also, our PCFR shows the state-of-the-art accuracy for node classification.

The key contribution of our work can be summarized as follows: 
(1) We propose a new concept of confidence and pseudo-confidence to represent the quality of a recovered feature.
(2) Based on the pseudo-confidence, we propose a novel feature recovery scheme with channel-wise between-node diffusion and node-wise between-channel propagation.
(3) PCFR achieves the state-of-the-art accuracy for node classification even at an extreme rate (e.g. 99.5\%) of missing features.

==> previous_version/3.1-0.tex <==
\subsection{Problem Setup}
\textbf{Notations.} An undirected graph is represented as $\mathcal{G} = (\mathcal{V}, \mathcal{E}, A)$ where $\mathcal{V}=\{v_i\}^N _{i=1}$ is the set of $N$ nodes, $\mathcal{E}$ is the edge set with $(v_i, v_j) \in \mathcal{E}$, and $A \in \mathbb{R}^{N \times N}$ denotes an adjacency matrix. $X = [x_{i,d}] \in \mathbb{R}^{N \times F}$ is a $F$-channel node feature matrix, i.e., $x_{i,d}$, $d$-th channel value of the node $v_i$. $\mathcal{N}(v_i)$ denotes the neighbors of $v_i$.
% neighbor 정의

% Further, we let $x_{i, *}$ denotes the $i$-th row vector of $X$ and $x_{*, d}$ denotes the $d$-th column vector of $X$.
% X를 원래의 의미를 더하기, 레이블
As we assume partial or even very few node features are known, we define $\mathcal{V}^{(d)}_k$ as the set of nodes on which the $d$-channel feature values are known.
We then refer to $\mathcal{V}^{(d)}_k$ as source nodes.
$V^{(d)}_u = V - V^{(d)}_k$ denotes the set of nodes on which the $d$-channel feature values are unknown. By reordering the nodes according to whether a feature value is known or not for $d$-th channel, we can write $d$-th channel graph signal and adjacency matrix as
\begin{equation*}
x^{(d)}=
\begin{bmatrix}
x^{(d)}_k\\
x^{(d)}_u
\end{bmatrix}
\qquad
A^{(d)} =
\begin{bmatrix}
A^{(d)}_{kk} & A^{(d)}_{ku} \\
A^{(d)}_{uk} & A^{(d)}_{uu}
\end{bmatrix}.
\end{equation*}
Here, $x^{(d)}$, $x^{(d)}_k$, and $x^{(d)}_u$ are column vectors that represent corresponding $d$-th channel graph signal. Since the graph is undirected, $A^{(d)}$ is symmetric and thus $(A^{(d)}_{ku})^\top = A^{(d)}_{uk}$. Note that $A^{(d)}$ is different from $A$ due to reordering while they represent the same graph structure.

% $X_k=\{(x_{i,d},i,d)\}$ denotes the set of triplets which are contained if and only if $d$-th channel value of $v_i$ is known.
\textbf{Learning on a graph with missing node features} is a transductive learning problem (typically node classification using GNN) where the structure of the graph $G$ is given while node features are partially known. In node classification, the partial label set $Y_L$ is given for the labeled node set $\mathcal{V}_L \in \mathcal{V}$. Then, the task is to infer the labels of the remaining unlabeled nodes based on the known features, the graph structure, and given label set.
Note that the aim of the task is to ensure the output on missing features is correct, not to recover the feature matrix accurately.
% 어떠한 node feature가 주어지는 graph-based task에 적용 가능하다. eg. node regression graph classification...
% existing approches homophily

% \textbf{Confidence-based Feature Reconstructor.}
% 본 논문에서 우리는 
% 우리는 node classification with missing node features를 해결하기 위해, X에 대한 추정치인 X hat을 reconstruct하고 X hat을 이용하여 뒤따르는 GNN을 학습한다. 우리가 제안하는 방법을 식으로 표현하면 다음과 같이 표현할 수 있다. f는 learning task와 독립적인 pre processing으로 취급될 수 있다. Note that 우리는 reconstruction이 아니라 ... . f는 homophily 가정 하에서 graph feature interpolation을 수행한다. f= f1 f2는 f1과 f2의 두 단계로 구성이 된다. g는 X^hat을 받아서 target task에 따라서 요구하는 output을 출력하는 GNN이다. Note that g로 어떠한 구조의 GNN도 사용할 수 있기에 node classification에만 제한되지 않고 다양한 task에 적용 가능하다.
% In this paper, we focus on different confidence in each information propagated from source nodes. Since homophily is a local property on a graph, a feature propagated from a known node inevitably become more uncertain as the distance from the node increases. To end this, we propose Confidence-based Feature Reconstructor (CFR), which utilizes approximated confidence based on shortest path distance from source nodes.
% 제안하는 framework에서
% In our proposed framework, CFR first estimate the full features $X$ as $\hat{X}$. We then train a GNN $g_\theta$ on the inferred fully-featured graph. Formally, proposed framework can be expressed as
% \begin{equation}
% \label{eq:problemsetup}
% \hat{X} = f(\,\{x^{(d)}_k\}^F_{d=1} \, , \; \{A^{(d)}\}^F_{d=1}\,)
% \quad \text{and} \quad
% \hat{Y} = g_\theta (\hat{X}, \,A)
% \end{equation}
% where $f$ represents CFR and $\hat{Y}$ is a prediction for desired output of a given task.
% Here, any GNN architecture can be adopted as $g_\theta$ depending on various tasks.

% Since two stages consisting CFR are both based on confidence, we first approximate confidence via shortest path distance from source nodes.
% As a first stage of CFR, features from source nodes diffuse to missing features on the basis of confidence.
% That is, intermediate estimate of full feature X is obtained after the diffusion. Then, we update this intermediate estimated features to a more accurate estimate by considering correlation between each channel.

% CFR는 두 단계로 구성된다.
% First of all, Confidence를 SPD from source nodes로 근사한다. (see Section 3.2)
% 첫 번째 단계는 ~이다. (see Section 3.3)
% 그리고 우리는 두번째 단계를 also based on(see Section 3.4)





% To tackle the aforementioned problem, we first reconstruct an estimate $\hat{X}$ of the full features $X$ with feature reconstructor $f$. Then, we train GNN $g$ using $\hat{X}$. Our proposed method can be expressed as 
% \begin{equation}
% \label{eq:problemsetup}
% \hat{X} = f(\,\{x^{(d)}_k\}^F_{d=1} \, , \; \{A^{(d)}\}^F_{d=1}\,)
% \quad \text{and} \quad
% \hat{Y} = g(\hat{X}, \,A)
% \end{equation}
% where $f$ is a feature reconstructor, $g$ is 

% $(\{ x^{(d)}_k\}^F_{d=1}, G, Y_L)$.
% To deal with graphs with unknown features, graph feature interpolation can be a reasonable solution. Graph feature interpolation is reconstructing the missing features with the graph structure and known features. The interpolation task requires some prior knowledge for the distribution of the features on the graph. Feature homophily is the most common assumption such that resulting reconstructed full features are smoothed.

% nder homophily assumption, we can estimate $\{ x^{(d)}_u\}^{(F)}_{d=1}$ based on $\{ x^{(d)}_k\}^F_{d=1}$ via graph feature interpolation.

%  목적은 feature estimate
% $\mathcal{V}_l$ is the labeled node set and would probably be different from or disjoint with $\mathcal{V}^d_k$. 



% Learning on a graph with missing node features는 그래프 G의 구조는 주어지며 label들과 node feature들을 부분적으로 알 수 있는 transductive learning problem이다. 우리는 이 문제를 graph feature interpolation을 통하여 해결하고자 한다. feature homophily라는 가장 공통된 가정을 바탕으로, full feature X에 대한 estimate인 X hat을 배우고자 한다. Specifically, 우리는 f(x_k, G) 

% 관사 체크
% 수식 위 아래 간격 줄이기
% Matrix에서 행 사이 간격 늘리기
% 필요 없는 부분 나중에 빼기
% 재정렬하는 내용 reordering

==> previous_version/3.1-1.tex <==
\subsection{Problem Setup}
\label{sub:problemsetup}
\textbf{Notations.} An undirected graph is represented as $\mathcal{G} = (\mathcal{V}, \mathcal{E}, A)$ where $\mathcal{V}=\{v_i\}^N _{i=1}$ is the set of $N$ nodes, $\mathcal{E}$ is the edge set with $(v_i, v_j) \in \mathcal{E}$, and $A \in \mathbb{R}^{N \times N}$ denotes an adjacency matrix. $X = [x_{i,d}] \in \mathbb{R}^{N \times F}$ is a $F$-channel node feature matrix, i.e., $x_{i,d}$, $d$-th channel value of the node $v_i$. $\mathcal{N}(v_i)$ denotes the set of neighbors of $v_i$. Given an arbitrary matrix $\mathbb{R}^{n \times m}$, we let $A_{i, :}$ denote the $i$-th row vector of A. Similarly, we let $A_{:, j}$ denote the $j$-th column vector of A.


As we assume partial or even very few node features are known, we define $\mathcal{V}^{(d)}_k$ as the set of nodes where the $d$-th channel feature values are known ($k$ in $\mathcal{V}^{(d)}_k$ means `known').
Then $\mathcal{V}^{(d)}_k$ is referred to as source nodes. The set of nodes with unknown $d$-th channel feature values is denoted by
$\mathcal{V}^{(d)}_u = \mathcal{V} - \mathcal{V}^{(d)}_k$. %denotes the set of nodes on which the $d$-th channel feature values are unknown. 
By reordering the nodes according to whether a feature value is known or not for $d$-th channel, we can write $d$-th channel graph signal and adjacency matrix as
\begin{equation*}
x^{(d)}=
\begin{bmatrix}
x^{(d)}_k\\
x^{(d)}_u
\end{bmatrix}
\qquad
A^{(d)} =
\begin{bmatrix}
A^{(d)}_{kk} & A^{(d)}_{ku} \\
A^{(d)}_{uk} & A^{(d)}_{uu}
\end{bmatrix}.
\end{equation*}
Here, $x^{(d)}$, $x^{(d)}_k$, and $x^{(d)}_u$ are column vectors that represent corresponding $d$-th channel graph signal. Since the graph is undirected, $A^{(d)}$ is symmetric and thus $(A^{(d)}_{ku})^\top = A^{(d)}_{uk}$. Note that $A^{(d)}$ is different from $A$ due to reordering while they represent the same graph structure.

\textbf{Learning on a graph with missing node features} can be an extension of the   transductive semi-supervised learning problem.
In contrast to the typical  semi-supervised learning given the complete node features, the missing node feature learning is done for node classification when both node features and node labels are partially known.
%using GNN where the structure of the graph $G$ is given while both node features and node labels are partially known. 
In node classification, the partial label set $Y_L$ is given for the labeled node set $\mathcal{V}_L \in \mathcal{V}$. Then, the task is to infer the labels of the remaining unlabeled nodes based on the known features, the graph structure, and given label set.
Note that the aim of our work is to achieve the best performance of a downstream task even for missing features, not to recover the complete feature matrix.

==> previous_version/3.1-2.tex <==
\subsection{Problem Statements}
missing feature recovery 에 대한 problem 설명, 기존 recovery 방법의 문제점 제시...
Unlike the existing approach, 
.....
우리의 접근 방법과 key idea, Overall Schematic 그림을 통해 전체 missing feature recovery scheme을 설명.

Notation은 표로 정리..


% \begin{table}
% \caption{Summary of notations used in the paper.}
% \label{notations}
% \centering
% {
% \begin{tabular}{cc|cc}
%      &  \\
%      & 
% \end{tabular}
% }
% \end{table}



\subsection{Problem Setup}
\label{sub:problemsetup}
\textbf{Notations.} An undirected graph is represented as $\mathcal{G} = (\mathcal{V}, \mathcal{E}, A)$ where $\mathcal{V}=\{v_i\}^N _{i=1}$ is the set of $N$ nodes, $\mathcal{E}$ is the edge set with $(v_i, v_j) \in \mathcal{E}$, and $A \in \{0,1\}^{N \times N}$ denotes an adjacency matrix. $X = [x_{i,d}] \in \mathbb{R}^{N \times F}$ is a $F$-channel node feature matrix, i.e., $x_{i,d}$, $d$-th channel value of the node $v_i$. $\mathcal{N}(v_i)$ denotes the set of neighbors of $v_i$. Given an arbitrary matrix $\mathbb{R}^{n \times m}$, we let $A_{i, :}$ denote the $i$-th row vector of A. Similarly, we let $A_{:, j}$ denote the $j$-th column vector of A. 

\input{tables/notation_table}

As we assume partial or even very few node features are known, we define $\mathcal{V}^{(d)}_k$ as the set of nodes where the $d$-th channel feature values are known ($k$ in $\mathcal{V}^{(d)}_k$ means `known'). The set of nodes with unknown $d$-th channel feature values is denoted by
$\mathcal{V}^{(d)}_u = \mathcal{V} \setminus \mathcal{V}^{(d)}_k$. Then $\mathcal{V}^{(d)}_k$ and $\mathcal{V}^{(d)}_u$ are referred to source nodes and missing nodes, repectively. By reordering the nodes according to whether a feature value is known or not for $d$-th channel, we can write $d$-th channel graph signal and adjacency matrix as
\begin{equation*}
x^{(d)}=
\begin{bmatrix}
x^{(d)}_k\\
x^{(d)}_u
\end{bmatrix}
\qquad
A^{(d)} =
\begin{bmatrix}
A^{(d)}_{kk} & A^{(d)}_{ku} \\
A^{(d)}_{uk} & A^{(d)}_{uu}
\end{bmatrix}.
\end{equation*}
Here, $x^{(d)}$, $x^{(d)}_k$, and $x^{(d)}_u$ are column vectors that represent corresponding $d$-th channel graph signal. Since the graph is undirected, $A^{(d)}$ is symmetric and thus $(A^{(d)}_{ku})^\top = A^{(d)}_{uk}$. Note that $A^{(d)}$ is different from $A$ due to reordering while they represent the same graph structure. $\bar{X} = [ \bar{x}_{i,d}]$ denotes some estimate of $X$ from $\{x^{(d)}_k\}^F_{d=1}$, $\{A^{(d)}\}^F_{d=1}$ with consideration of homophily.

\textbf{Learning on a graph with missing node features} can be an extension of the transductive semi-supervised learning problem.
In contrast to the typical  semi-supervised learning given the complete node features, the missing node feature learning is done for node classification when both node features and node labels are partially known.
%using GNN where the structure of the graph $G$ is given while both node features and node labels are partially known. 
In node classification, the partial label set $Y_L$ is given for the labeled node set $\mathcal{V}_L \in \mathcal{V}$. Then, the task is to infer the labels of the remaining unlabeled nodes based on the known features, the graph structure, and given label set.
Note that the aim of our work is to achieve the best performance of a downstream task even for missing features, not to recover the complete feature matrix.

==> previous_version/3.2-0.tex <==




\subsection{Overview}
\label{sub:overview}


Since homophily is a local property on a graph, %information propagated 
message passing  strength from a source node inevitably is attenuated %become %more uncertain 
as the distance from the source node increases.
Thus, we focus on this different confidence in each information propagated 
from source nodes.
In this paper, we propose Confidence-Based Feature Reconstructor (CBFR), which utilizes approximated confidence based on shortest path distance (SPD) from source nodes.

In our proposed framework, CBFR first estimate the full features $X$ as $\hat{X}$. We then train a GNN $g_\theta$ on the inferred fully-featured graph. Formally, proposed framework can be expressed as
\begin{equation}
\label{eq:problemsetup}
\hat{X} = f(\,\{x^{(d)}_k\}^F_{d=1} \, , \; \{A^{(d)}\}^F_{d=1}\,)
\quad \text{and} \quad
\hat{Y} = g_\theta (\hat{X}, \,A)
\end{equation}
where $f$ represents CBFR and $\hat{Y}$ is a prediction for desired output of a given task.
Here, any GNN architecture can be adopted as $g_\theta$ according to a task.
% Since two stages consisting CBFR are both based on confidence, we first approximate confidence via shortest path distance from source nodes (see Section~\ref{sub:SPDSN}).
Since two stages constituting CBFR are both based on confidence, we first approximate confidence in each node feature via SPD from source nodes (see Section~\ref{sub:SPDSN}).
As a first stage of CBFR, features from source nodes diffuse to missing features on the basis of the approximated confidence (see Section~\ref{sub:CFD}).
$\Tilde{X}$ which denotes an intermediate estimate of full feature X is obtained after the diffusion. Then, we update this intermediate estimated features $\Tilde{X}$ to a more accurate estimate $\hat{X}$ by considering correlation between each channel. (see Section~\ref{sub:FUCC}).

==> previous_version/3.2-1.tex <==




\subsection{EC-based feature recovery}
\label{sub:overview}

%First of all, we define confidence which is a key concept in this paper.
%Since homophily is a local property on a graph,
%similarity between two nodes tends to decrease as distance between the two nodes increase.

Our goal is to recover a missing feature of a node from the given features of source nodes in $\mathcal{G}$. To this end, we introduce a concept of confidence on a recovered feature in a node. To estimate the confidence, we first define SPDS(shortest path distance from source nodes) of a missing node, defined in Definition 1. 

\begin{definition} \label{definition2}
SPDS(shortest path distance from source nodes) is defined by the shortest path distance to a node from its nearest source node for each channel.
\end{definition}

According to Definition 1, 
SPDS of $i$-th node for $d$-th channel is denoted by $S_{i,d}$ which is calculated by \begin{equation}
\label{eq:problemsetup}
S_{i,d}=s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})\,,
\end{equation}
where $s(\cdot)$ yields the number of the shortest hops between $i$-th node and its nearest source node in 
$\mathcal{V}^{(d)}_k$ on $A^{(d)}$. Note that if $i$-th node is a source node, its nearest source node is itself, thus $S_{i,d}$ becomes zero.
we construct SPH matrix $S \in \mathbb{R}^{N \times F}$ of which elements are $S_{i,d}$.

Based on homophily that is a local property on a graph, the feature similarity between any two nodes tends to increase as the number of shortest hops between the two nodes decreases. Thus we assume that a recovered feature $\hat{x}_{i,d}$ of a missing node with smaller SPDS becomes more confident. 

That is. as distance from the nearest source node in $ \mathcal{V}^{(d)}_k$ to $v_i$ decreases, $\bar{x}_{i,d}$ probably becomes more accurate. Confidence in $\bar{x}_{i,d}$ is defined as expected similarity between $\bar{x}_{i,d}$ and true value $x_{i,d}$, which is a value between 0 and 1. Since estimate for $x^{(d)}_k$ should be the given true feature values, confidence in all $\bar{x}_{i,d}$ for $x^{(d)}_k$ is 1. When $\bar{x}_{i,d}$ estimates a feature value in $x^{(d)}_u$, confidence in $\bar{x}_{i,d}$ will decrease towards 0 as distances from source nodes to $v_i$ increases. We can express defined confidence as a function $\rho :\mathbb{R} \rightarrow \mathbb{R}$ as follows:
%\newtheorem{definition1}{Definition}
\begin{definition} \label{definition1}
We define confidence 
in $\bar{x}_{i,d}$ by a function $\rho(\bar{x}_{i,d}|\mathcal{V}^{d}_k , A^{(d)})$ which outputs expected similarity between $\bar{x}_{i,d}$ and $\bar{x}_{i,d}$.
\end{definition}

We focus on this newly defined concept, confidence to reconstruct missing features accurately.

We propose Confidence-Based Feature Reconstructor (CBFR), which utilizes approximated confidence based on shortest path distance (SPD) from source nodes. In our proposed framework, CBFR first estimate the full features $X$ as $\hat{X}$. We then train a GNN $g_\theta$ on the inferred fully-featured graph. Formally, the proposed framework can be expressed as
\begin{equation}
\label{eq:problemsetup}
\hat{X} = f(\,\{x^{(d)}_k\}^F_{d=1} \, , \; \{A^{(d)}\}^F_{d=1}\,)
\quad \text{and} \quad
\hat{Y} = g_\theta (\hat{X}, \,A)
\end{equation}
where $f$ represents CBFR and $\hat{Y}$ is a prediction for desired output of a given task.
Here, any GNN architecture can be adopted as $g_\theta$ according to a task.
Since two stages constituting CBFR are both based on confidence, we first approximate confidence in each node feature via SPD from source nodes (see Section~\ref{sub:SPDSN}).
As a first stage of CBFR, features from source nodes diffuse to missing features on the basis of the approximated confidence (see Section~\ref{sub:CFD}).
$\Tilde{X}$ which denotes an intermediate estimate of full feature X is obtained after the diffusion. Then, we update this intermediate estimated features $\Tilde{X}$ to a more accurate estimate $\hat{X}$ by considering correlation between each channel. (see Section~\ref{sub:FUCC}).

% Then, propagation from source nodes under homophily.
% of $x_{i,d}$ as degree of predicted similarity between true value for $x_{i,d}$ and inferred value for $x_{i,d}$ via $x^{(d)}_k$.
% Since homophily is a local property on a graph,
% similarity between two nodes tends to decrease as distance between the two nodes increase. Therefore,
% confidence가 source node, missing node 
% Therefore, when a unknown node receives feature from a source node 일련의 propagation을 통해서, 
% 그러므로, missing feature를 가진 노드가 source node로 
% a feature propagated from a source node inevitably become more uncertain as the distance from the node increases.
%
% Since homophily is a local property on a graph, %information propagated 
% message passing  strength from a source node inevitably is attenuated %become %more uncertain 
% as the distance from the source node increases.
% Thus, we focus on this message passing  strength depending on the distance 
%in each information propagated 
% from source nodes.

==> previous_version/3.3-0.tex <==
\subsection{Confidence Approximation Based on SPD from Source Nodes}
\label{sub:SPDSN}


% criterion, working principle
% 척도가 될 수 있다

In this section, we present a novel approximation method for confidence in each inferred node feature by using the shortest path distance (SPD) of each node defined in Definition 2. 

\begin{definition} \label{definition2}
SPD(shortest path distance) is defined by a distance via the shortest path to a non-source node  from its nearest source node for each channel, i.e., SPD of $i$-th node for $d$-th channel is denoted by $S_{i,d}$ which is calculated by \begin{equation}
\label{eq:problemsetup}
S_{i,d}=s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})\,,
\end{equation}
where $s(\cdot)$ yields the number of the shortest hops between $i$-th node and its nearest source node   in 
$\mathcal{V}^{(d)}_k$ on $A^{(d)}$. Note that if $i$-th node is a source node, its nearest source node is itself, thus $S_{i,d}$ becomes zero.
\end{definition}

According to Definition 1, we construct SPD matrix $S \in \mathbb{R}^{N \times F}$ of which elements are $S_{i,d}$.

Since confidence in $\bar{x}_{i,d}$ decreases as distances from source nodes increases, we approximate confidence in $\bar{x}_{i,d}$ by using the shortest path distance (SPD) from source nodes $\mathcal{V}^{(d)}_k$ to $v_i$.


% The crucial working principle is that 

% SPD matrix 정의
% 이 함수를 이용하여 S, 모든 채널에 대하여 모든 노드의 출력이 담긴 행렬 S를 정의한다.
% S는 다음과 같이 정의된다. S =\in N \times F, S_i,d = $s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})=0$
% 즉 S의 each row는 특정 노드의 각 채널들에 대한 SPD from source nodes를 의미.
% S의 each column는 특정한 채널에서 각 노드의 SPD from source nodes를 의미한다.
We define SPD from source nodes for $d$-th channel as a function $s(\,\cdot\, |\mathcal{V}^{(d)}_k, A^{(d)}):\mathcal{V} \rightarrow \mathbb(\{0\} \cup {Z}^+)$. Since SPD from a source node to source nodes is zero, $s$ outputs zero only for a source node, That is, $s(v_i |\mathcal{V}^{(d)}_k, A^{(d)})=0$ for all $v_i \in \mathcal{V}^{(d)}_k$ while $s$ outputs a positive integer for a missing node, i.e., $s(v_i |\mathcal{V}^{(d)}_k, A^{(d)}) \in \mathbb{Z}^+$ for all $v_i \in \mathcal{V}^{(d)}_u$. We then construct a matrix $S \in \mathbb{R}^{N \times F}$ which consists of all output of the function $s$ for each estimated node feature. $S$ is defined as $[S_{i,d}]$. Then, $S_{i,:}$ denotes SPD vector of which element represents SPD from source nodes to an $i$-th node for each channel and $S_{:,d}$ denotes SPD vector of which element represents SPD from source nodes to each node for $d$-th channel.

We approximate confidence of $\bar{x}_{i,d}$ by $\alpha^{s(v_i |\mathcal{V}^{(d)}_k, A^{(d)})} \,(0 < \alpha < 1)$, where $\alpha$ is a hyperparameter. By doing so, approximated confidence is 1 for source nodes. Also, approximated confidence for a missing node decreases exponentially as distances from source nodes increases. Likewise, our approximation method reflects well the tendency of confidence. Since both two stages constituting CBFR leverages this confidence approximation based on SPD from source nodes, $S$ plays a important role as a lookup table.


% We 근사한다 u 에서 연결되어 있는 이웃들에 대한 confidence를 다음과 같이
% where delta는 0과 1 사이의 값을 갖는 어떠한 hyperameter라고 하자.
% 자신보다 상대적으로 source node와 더 가까운 노드에 대해서는, node에 대한 confidence는 1로 정한다.
% 그리고 자신과 source node로부터 SPD가 가까운 이웃 노드에 대한 confidence는 delta로 근사한다.
% 자신보다 source node로부터 SPD가 먼 이웃에 대한 confidence는 detla^2로 근사한다.
% 즉, 자기 자신과의 상대적 SPD from source nodes 우위를 비교하여, 그 값 클 수록 더 작은 값의 근사된 confidence를 할당한다.
% first step인 Diffusion 과 second step인 update 과정에 모두 관여하는 이 근사 방법은 CBFR에게 매우 중요한 요소이다. 

% 아래의 내용은 조금 더 정돈하여 작성하겠습니다.
% $\textbf{Theorem 1.}$ Given an arbitrary node $v_j$ and suppose $s(v_j|\mathcal{V}^{(d)}_k, A^{(d)})=m$. $s(v_i|\mathcal{V}^{(d)}_k, A^{(d)}) \in \{m-1,m,m+1\} \; \, \text{for} \, \; v_i \in \mathcal{N}(v_j).$
% Therefore, $s(v_i|\mathcal{V}^{(d)}_k, A^{(d)}) - s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})$

% a node with missing $d$-th channel feature 의 관점에서 보도록 하자.
% 만약 그 노드에 해당하는 S의 값이 m이라고 하자.
% 그럼 그 노드의 이웃이 가질 수 있는 S 값은 m-1, m or m+1 뿐이다.
% 즉, 수식으로.
% 한 가지 예로, s가 2인 노드는 SPD가 2이기 때문에 source node과 직접적으로 연결 될 수 없다. s가 2인 노드와 연결되어 있는 이웃들의 s 출력은 1,2,3 만이 가능하다.
% 이에 대한 증명은 Appendix에 있다.

% We 근사한다 u 에서 연결되어 있는 이웃들에 대한 confidence를 다음과 같이
% where delta는 0과 1 사이의 값을 갖는 어떠한 hyperameter라고 하자.
% 자신보다 상대적으로 source node와 더 가까운 노드에 대해서는, node에 대한 confidence는 1로 정한다.
% 그리고 자신과 source node로부터 SPD가 가까운 이웃 노드에 대한 confidence는 delta로 근사한다.
% 자신보다 source node로부터 SPD가 먼 이웃에 대한 confidence는 detla^2로 근사한다.
% 즉, 자기 자신과의 상대적 SPD from source nodes 우위를 비교하여, 그 값 클 수록 더 작은 값의 근사된 confidence를 할당한다.
% first step인 Diffusion 과 second step인 update 과정에 모두 관여하는 이 근사 방법은 CBFR에게 매우 중요한 요소이다. 

% At CBFR, first stage in Section 3.4 와 second stage in Section 3.5은 이러한 이 approximation method로 구한 S를 기반으로 한다.


% 근사하는 방법. 연결 가능한 가짓수, 증명 필요?

% Since SPD from a source node to source nodes is 0 (distance to itself), 
% $s(\,\cdot\, |\mathcal{V}^{(d)}_k, A^{(d)})$ outputs 0 for every source node in $d$-th channel, and outputs a positive integer for a node with missing $d$-th channel feature. That is, $s(u|\mathcal{V}^{(d)}_k, A^{(d)})=0$ for all $u \in \mathcal{V}^{(d)}_k$ while $s(u|\mathcal{V}^{(d)}_u, A^{(d)}) \in \mathbb{Z}^+$ for all $u \in \mathcal{V}^{(u)}_k$.









% 연결 가능한 가짓수, 증명 필요?

% 함수에 대한 정의 s

% 

% 4.4, 4.5에서 이 matrix 계속 지정하려면 Matrix row/column vector notation 추가해야 될 것 같은데?

% given graph?? 넣어줘야?

==> previous_version/3.3-1.tex <==
\subsection{Confidence Approximation Based on SPD from Source Nodes}
\label{sub:SPDSN}




In this section, we present a novel approximation method for confidence in each inferred node feature by using the shortest path distance (SPD) of each node defined in Definition 2.

\newtheorem{definition}{Definition}
\label{definition3}
\begin{definition}
SPD(shortest path distance) is defined by a distance via the shortest path to a non-source node  from its nearest source node for each channel, i.e., SPD of $i$-th node for $d$-th channel is denoted by $S_{i,d}$ which is calculated by \begin{equation}
\label{eq:problemsetup}
S_{i,d}=s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})\,,
\end{equation}
where $s(\cdot)$ yields the number of the shortest hops between $i$-th node and its nearest source node   in 
$\mathcal{V}^{(d)}_k$ on $A^{(d)}$. Note that if $i$-th node is a source node, its nearest source node is itself, thus $S_{i,d}$ becomes zero.
\end{definition}

According to Definition 3, we construct SPD matrix $S \in \mathbb{R}^{N \times F}$ of which elements are $S_{i,d}$.

Since confidence in $\bar{x}_{i,d}$ decreases as distances from source nodes increases, we approximate confidence in $\bar{x}_{i,d}$ by using the shortest path distance (SPD) from source nodes $\mathcal{V}^{(d)}_k$ to $v_i$.


% The crucial working principle is that 

% SPD matrix 정의
% 이 함수를 이용하여 S, 모든 채널에 대하여 모든 노드의 출력이 담긴 행렬 S를 정의한다.
% S는 다음과 같이 정의된다. S =\in N \times F, S_i,d = $s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})=0$
% 즉 S의 each row는 특정 노드의 각 채널들에 대한 SPD from source nodes를 의미.
% S의 each column는 특정한 채널에서 각 노드의 SPD from source nodes를 의미한다.
We define SPD from source nodes for $d$-th channel as a function $s(\,\cdot\, |\mathcal{V}^{(d)}_k, A^{(d)}):\mathcal{V} \rightarrow \mathbb(\{0\} \cup \mathbb{Z}^+)$. Since SPD from a source node to source nodes is zero, $s$ outputs zero only for a source node, That is, $s(v_i |\mathcal{V}^{(d)}_k, A^{(d)})=0$ for all $v_i \in \mathcal{V}^{(d)}_k$ while $s$ outputs a positive integer for a missing node, i.e., $s(v_i |\mathcal{V}^{(d)}_k, A^{(d)}) \in \mathbb{Z}^+$ for all $v_i \in \mathcal{V}^{(d)}_u$. We then construct a matrix $S \in \mathbb{R}^{N \times F}$ which consists of all output of the function $s$ for each estimated node feature. $S$ is defined as $[S_{i,d}]$. Then, $S_{i,:}$ denotes SPD vector of which element represents SPD from source nodes to an $i$-th node for each channel and $S_{:,d}$ denotes SPD vector of which element represents SPD from source nodes to each node for $d$-th channel.

We approximate confidence in $\bar{x}_{i,d}$ as follows:
\newtheorem{definition3}{Definition}
\label{definition4}
\begin{definition}
Approximated confidence $\hat{\rho} : \mathbb{R} \rightarrow \mathbb{R}$ is defined by $\hat{\rho}(\bar{x}_{i,d}|\mathcal{V}^{d}_k , A^{(d)})= \alpha^{s(v_i |\mathcal{V}^{(d)}_k, A^{(d)})}$ where $\alpha$ is a hyperparameter in the range $[0,1]$.
\end{definition}
By Definition 4, approximated confidence is 1 for source nodes. Also, approximated confidence for a missing node decreases exponentially as distances from source nodes increases. Likewise, our approximation method reflects well the tendency of confidence.

Since both two stages constituting CBFR leverages this confidence approximation based on SPD from source nodes, $S$ plays a important role as a lookup table.


% We 근사한다 u 에서 연결되어 있는 이웃들에 대한 confidence를 다음과 같이
% where delta는 0과 1 사이의 값을 갖는 어떠한 hyperameter라고 하자.
% 자신보다 상대적으로 source node와 더 가까운 노드에 대해서는, node에 대한 confidence는 1로 정한다.
% 그리고 자신과 source node로부터 SPD가 가까운 이웃 노드에 대한 confidence는 delta로 근사한다.
% 자신보다 source node로부터 SPD가 먼 이웃에 대한 confidence는 detla^2로 근사한다.
% 즉, 자기 자신과의 상대적 SPD from source nodes 우위를 비교하여, 그 값 클 수록 더 작은 값의 근사된 confidence를 할당한다.
% first step인 Diffusion 과 second step인 update 과정에 모두 관여하는 이 근사 방법은 CBFR에게 매우 중요한 요소이다. 

% 아래의 내용은 조금 더 정돈하여 작성하겠습니다.
% $\textbf{Theorem 1.}$ Given an arbitrary node $v_j$ and suppose $s(v_j|\mathcal{V}^{(d)}_k, A^{(d)})=m$. $s(v_i|\mathcal{V}^{(d)}_k, A^{(d)}) \in \{m-1,m,m+1\} \; \, \text{for} \, \; v_i \in \mathcal{N}(v_j).$
% Therefore, $s(v_i|\mathcal{V}^{(d)}_k, A^{(d)}) - s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})$

% a node with missing $d$-th channel feature 의 관점에서 보도록 하자.
% 만약 그 노드에 해당하는 S의 값이 m이라고 하자.
% 그럼 그 노드의 이웃이 가질 수 있는 S 값은 m-1, m or m+1 뿐이다.
% 즉, 수식으로.
% 한 가지 예로, s가 2인 노드는 SPD가 2이기 때문에 source node과 직접적으로 연결 될 수 없다. s가 2인 노드와 연결되어 있는 이웃들의 s 출력은 1,2,3 만이 가능하다.
% 이에 대한 증명은 Appendix에 있다.

% We 근사한다 u 에서 연결되어 있는 이웃들에 대한 confidence를 다음과 같이
% where delta는 0과 1 사이의 값을 갖는 어떠한 hyperameter라고 하자.
% 자신보다 상대적으로 source node와 더 가까운 노드에 대해서는, node에 대한 confidence는 1로 정한다.
% 그리고 자신과 source node로부터 SPD가 가까운 이웃 노드에 대한 confidence는 delta로 근사한다.
% 자신보다 source node로부터 SPD가 먼 이웃에 대한 confidence는 detla^2로 근사한다.
% 즉, 자기 자신과의 상대적 SPD from source nodes 우위를 비교하여, 그 값 클 수록 더 작은 값의 근사된 confidence를 할당한다.
% first step인 Diffusion 과 second step인 update 과정에 모두 관여하는 이 근사 방법은 CBFR에게 매우 중요한 요소이다. 

% At CBFR, first stage in Section 3.4 와 second stage in Section 3.5은 이러한 이 approximation method로 구한 S를 기반으로 한다.


% 근사하는 방법. 연결 가능한 가짓수, 증명 필요?

% Since SPD from a source node to source nodes is 0 (distance to itself), 
% $s(\,\cdot\, |\mathcal{V}^{(d)}_k, A^{(d)})$ outputs 0 for every source node in $d$-th channel, and outputs a positive integer for a node with missing $d$-th channel feature. That is, $s(u|\mathcal{V}^{(d)}_k, A^{(d)})=0$ for all $u \in \mathcal{V}^{(d)}_k$ while $s(u|\mathcal{V}^{(d)}_u, A^{(d)}) \in \mathbb{Z}^+$ for all $u \in \mathcal{V}^{(u)}_k$.









% 연결 가능한 가짓수, 증명 필요?

% 함수에 대한 정의 s

% 

% 4.4, 4.5에서 이 matrix 계속 지정하려면 Matrix row/column vector notation 추가해야 될 것 같은데?

% given graph?? 넣어줘야?

==> previous_version/3.3-2.tex <==
\subsection{Confidence Approximation Based on SPD from Source Nodes}
\label{sub:SPDSN}




In this section, we present a novel approximation method for confidence in each inferred node feature by using the shortest path distance (SPD) of each node defined in Definition 2.



We define SPD from source nodes for $d$-th channel as a function $s(\,\cdot\, |\mathcal{V}^{(d)}_k, A^{(d)}):\mathcal{V} \rightarrow \mathbb(\{0\} \cup \mathbb{Z}^+)$. Since SPD from a source node to source nodes is zero, $s$ outputs zero only for a source node, That is, $s(v_i |\mathcal{V}^{(d)}_k, A^{(d)})=0$ for all $v_i \in \mathcal{V}^{(d)}_k$ while $s$ outputs a positive integer for a missing node, i.e., $s(v_i |\mathcal{V}^{(d)}_k, A^{(d)}) \in \mathbb{Z}^+$ for all $v_i \in \mathcal{V}^{(d)}_u$. We then construct a matrix $S \in \mathbb{R}^{N \times F}$ which consists of all output of the function $s$ for each estimated node feature. $S$ is defined as $[S_{i,d}]$. Then, $S_{i,:}$ denotes SPD vector of which element represents SPD from source nodes to an $i$-th node for each channel and $S_{:,d}$ denotes SPD vector of which element represents SPD from source nodes to each node for $d$-th channel.

We approximate confidence in $\bar{x}_{i,d}$ as follows:
\newtheorem{definition3}{Definition}
\label{definition4}
\begin{definition}
Approximated confidence $\hat{\rho} : \mathbb{R} \rightarrow \mathbb{R}$ is defined by $\hat{\rho}(\bar{x}_{i,d}|\mathcal{V}^{d}_k , A^{(d)})= \alpha^{s(v_i |\mathcal{V}^{(d)}_k, A^{(d)})}$ where $\alpha$ is a hyperparameter in the range $[0,1]$.
\end{definition}
By Definition 4, approximated confidence is 1 for source nodes. Also, approximated confidence for a missing node decreases exponentially as distances from source nodes increases. Likewise, our approximation method reflects well the tendency of confidence.

Since both two stages constituting CBFR leverages this confidence approximation based on SPD from source nodes, $S$ plays a important role as a lookup table.

==> previous_version/3.4-0.tex <==
\subsection{Confidence-Based Feature Diffusion}
\label{sub:CFD}

In this section, we present a first stage of CBFR, confidence-based feature diffusion. Confidence-based feature diffusion diffuses features with different edge weight depending on approximated confidence in each node feature.

% Diffusion is a process that consists of iterative propagation, which can be expressed as iteratively multiplying a feature matrix by a transition matrix.

As feature diffusion starts, source nodes start propagating their features to their neighbors for each channel independently. While source nodes keep their features that are true values, missing nodes aggregate features from connected nodes. Missing nodes aggregate inaccurate tentative features from other connected missing nodes in addition to features from source nodes. By considering both homophily and confidence which is an essential concept for missing features setting, We design a weighted adjacency matrix for feature diffusion.
% 이를 위해서 우리는 상대적인 approximated confidence를 다음과 같이 정의한다.
Our design objective is that a missing node aggregate more features from node features with high approximated confidence. To this end, we consider approximated confidence in features for neighboring nodes of a specific missing feature.

Consider a missing node $v_i$ and $v_j \in \mathcal{N}(v_i)$. Since a distance between $v_i$ and $v_j$ is 1, difference between outputs of $s$ for the two nodes cannot exceed 1. Formally, This observation can be expressed as the following theorem with proof in Appendix. 
\newtheorem{theorem}
\label{theorem1}
\begin{theorem}
Given a node $v_i$ s.t. $s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})=m\geq1$. Then, $s(v_j|\mathcal{V}^{(d)}_k, A^{(d)}) \in \{m-1,m,m+1\}$ for $v_j \in \mathcal{N}(v_i).$ Otherwise, if $v_i$ s.t. $s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})=0$ is given, $s(v_j|\mathcal{V}^{(d)}_k, A^{(d)}) \in \{0,1\}$ for $v_j \in \mathcal{N}(v_i).$
\end{theorem}
From Theorem 1, the following corollary holds trivially.

\begin{corollary}
If $s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})=m\geq1$, then \ $s(v_j|\mathcal{V}^{(d)}_k, A^{(d)})-s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})  \in \{-1,0,1\}$ for $v_j \in \mathcal{N}(v_i)$. Otherwise, if $s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})=0$, then $s(v_j|\mathcal{V}^{(d)}_k, A^{(d)})-s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})  \in \{0,1\}$ for $v_j \in \mathcal{N}(v_i)$.
\end{corollary}

Theorem 1 shows that from any node, there are at most three possible cases for output of $s$ for its neighbors.
We then define relative approximated confidence $\hat{\rho}_{r}$, a function to output relative amount of approximated confidence in a particular node feature compared to other node features as follows:
\newtheorem{definition5}{Definition}
\label{definition5}
\begin{definition}
Relative approximated confidence in $\bar{x}_{i,d}$ to $\bar{x}_{j,d}$ is define by $\hat{\rho}_{r} (\bar{x}_{i,d}| \bar{x}_{j,d}) = \hat{\rho}(\bar{x}_{i,d}|\mathcal{V}^{d}_k , A^{(d)}) / \hat{\rho}(\bar{x}_{j,d}|\mathcal{V}^{d}_k , A^{(d)})$.
\end{definition}

By Definition 4, we can rewrite $\hat{\rho}_{r} (\bar{x}_{i,d}| \bar{x}_{j,d})$ as $\alpha^{s(v_j|\mathcal{V}^{(d)}_k, A^{(d)})-s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})}$. Then, according to Corollary 1, the following corollary also holds.


\begin{corollary}
If $s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})=m\geq1$, then $\hat{\rho}_{r} (\bar{x}_{i,d}| \bar{x}_{j,d}) \in \{\alpha^{-1}, 1, \alpha\}\,$ for $v_j \in \mathcal{N}(v_i)$.
\end{corollary}

Corollary 1.2 shows that at the point of view of a missing node, there are only three possible cases for relative approximated confidence in its neighboring feature to its feature, while two cases for a source node.

Before constructing a weighted adjacency matrix based on approximated confidence, we reorder nodes according to whether a feature value is known or not for $d$-channel as in $A^{(d)}$. After feature diffusion, we order the nodes according to the original numbering.

Let $\tilde{X}=[\tilde{x}_{i,d}]$ denote an estimate of full feature $X$, which is updated via propagation steps in confidence-based feature diffusion. We then construct weighted adjacency matrix $W^{(d)}$ for $d$-th channel with $\alpha_1$ for a hyperparameter $\alpha$. $W^{(d)} \in \mathbb{R}^{N \times N}$ is defined as follows,
\begin{equation}
    W^{(d)}_{i,j} = \begin{cases} \hat{\rho}_{r} (\tilde{x}_{i,d}| \tilde{x}_{j,d}) =  \alpha^{s(v_j|\mathcal{V}^{(d)}_k, A^{(d)})-s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})} & \,\text{if} \; i \neq j \, , \, A^{(d)}_{i,j} = 1
    \\
    0 & \,\text{if} \; i \neq j \, , \, A^{(d)}_{i,j} = 0
    \\
    1 & \,\text{if} \; i = j
    \end{cases}
\end{equation}

Note that self-loops are added to $W^{d}$ with weight 1 so that each node can keep some of its own feature. We design $W^{d}$ with the aim of allowing $\tilde{x}_{i,d}$ to aggregate more features with high confidence from its neighbors. According to Corollary 1.2, $W_{i,j} \in \{\alpha^{-1}, 0, \alpha\}$ when $v_i$ and $v_j$ are connected.
% 추가
% Note that A는 symmtric하지 않으며, A_ij와 Aji의 곱은 1이 된다. 이는 A_ij가 alpha이면 A_ji는 alpha^-1이 되는 것을 의미한다. 반대로 A_ij가 alpha^-1이면 A_ij는 alpha가 된다. A_ij는 node i가 node j로 부터 받아오는 것에 대응되는 edge weight를 의미한다. 따라서 두 노드의 AP(v_i)>AP(v_j)일 때, confidence가 더 높은 v_i는 v_j로 더 많은 feature를 전파할 수 있도록 한다 while v_i는 v_j로부터 적은 feature를 받아온다.

To ensure convergence of diffusion process, we then define $\hat{W}^{(d)} =(D^{(d)})^{-1} W^{(d)}$ through row-stochastic normalization with $D^{(d)}_{ii} = \Sigma_j W_{i,j}$.
Since $x^{d}_k$ with true feature values should be preserved, we replace first $|\mathcal{V}^{(d)}|$ rows of $\hat{W}$ with one-hot vectors indicating $\mathcal{V}^{(d)}_k$.
a transition matrix $\tilde{W}$ can be expressed as
\begin{equation}
    \tilde{W} = \begin{bmatrix}
\textbf{I} & \textbf{0} \\
\hat{W}^{(d)}_{uk} & \hat{W}^{(d)}_{uu}
\end{bmatrix}.
\end{equation}
Note that $\tilde{W}$ is still row-stochastic.
An aggregation in a specific node can be regarded as a weighted sum of features on neighboring nodes. A row-stochastic matrix for transition matrix means that when a node aggregates features from its neighbors, the sum of the weights is 1. Therefore, unlike symmetric or column-stochastic (random walk) transition matrix, features of missing nodes can be formed at the same scale of known features.

For diffusion, we initialize missing feature values $x^{(d)}_u$ to zero. Now, We define K-steps Confidence-based feature diffusion as
\begin{equation}
\begin{split}
   &\tilde{x}^{(d)} (t) = \tilde{W}\, \tilde{x}^{(d)} (t-1)\\&
\tilde{x}^{(d)} (K) = \tilde{W}^K \tilde{x}(0)
\end{split}
\end{equation}
where $\tilde{x}^{(d)} (t)$ denotes estimate for ${x}^{(d)}$ after t-steps diffusion.
% diffusion을 명확히. K step의 propagation

% As diffusion proceeds, 

% 다 끝난 X(K)를 다시 원래 order로 돌려서 concate nate
% 그리고 다음 stage로 갈 큰 행렬 형성.

% 또한 

% If we multiply $W$ by a node feature matrix, $W_{i,j}$ correspond to propagation from $v_j$ to $v_i$.
% Consider propagation with $W$ between connected nodes $v_i$ and $v_j$.
% Since $\hat{\rho}_{r} (\tilde{x}_{i,d}| \tilde{x}_{j,d})= (\hat{\rho}_{r} (\tilde{x}_{j,d}| \tilde{x}_{i,d}))^{-1}$ by Definition 5, $W_{i,j}=W_{j,i}^{-1}$. Consider propagation between connected nodes $v_i$ and $v_j$. If $W_{i,j}$ = 




% 새롭게 형성되는 feature의 scale을 고려했을 때. row stochastic.
% x^{(0)}에 대한 정의. step
% 채널에 따라 독립적이다.

% We design $W$ with the aim of allowing $\tilde{x}_{i,d}$ to aggregate more features with high confidence from its neighbors. If we multiply $W$ by a node feature matrix, $W_{i,j}$ correspond to propagation from $v_j$ to $v_i$.
% According to Corollary 1.2, $W_{i,j} \in \{\alpha^{-1}, 0, \alpha\}$ when $v_i$ and $v_j$ are connected. Since $\hat{\rho}_{r} (\tilde{x}_{i,d}| \tilde{x}_{j,d})= (\hat{\rho}_{r} (\tilde{x}_{j,d}| \tilde{x}_{i,d}))^{-1}$ by Definition 5, $W_{i,j}=W_{j,i}^{-1}$. Consider propagation between connected nodes $v_i$ and $v_j$. If $W_{i,j}$


% initialize는 missing은 0으로


% 일단 여기까지 작성하고 정리

% 수렴성을 위하여 Adjacency를 다음과 같이 normalize하게 된다.
% [I 0 A A] 배치.
% eq with bar
% random walk style. column stochastic.
% Confidence-Based Feature Diffusion은 다음과 같은 일련의 propagation을 통해서 수행된다.

% \bar a는 confidence를 고려하였다.

% Note that CBFD는 채널에 대해서 독립적으로 이루어진다.

% According to Corollary~\ref{corollary}, relative approximated confidence of a missing node to its each neighbor is in $\{\alpha^{-1},1,\alpha\}$. 
% We use $\alpha_1$ as $\alpha$ for confidence-based feature diffusion.



% homophily라는 가정 하에서, missing node의 feature는 이웃들의 feature를 통해서 diffusion을 통하여 채운다. (일련의 propagation.)


% 우리의 디자인 목적은 a missing node feature가 aggregation 단계에서 자신보다 더 신뢰할 수 있는 노드로 부터는 더 받아 오고, 상대 신뢰도가 더 적을 수록 덜 받아오도록 하는 것이다.
% 이를 가능하게 하기 위해, 우리는 confidence-based weighted adjacency matrix, A_alpha.를 다음과 같이 정의한다.
% 그리고 수렴성을 보장하기 위하여 A_alpha를 column stochastic하게 normalized. D 사용하여 표현.

% numbering issue 해결하기

% missing node 
% 각기 다른 weight로 diffusion


% Relative confidence 
% $s(v_j|\mathcal{V}^{(d)}_k, A^{(d)})-s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})$


% 에너지
% 수렴성을 보장하기 위해서
% 수렴안 하는 이유

% X tilde
 % concatenate 하고 원래의 order로 맞추어 feature들을 concatenate. X. 즉 matrix의 형태로.
 
%  across the node
% deviate from symmetric

% 자신보다 상대적으로 source node와 더 가까운 노드에 대해서는, node에 대한 confidence는 1로 정한다.
% 그리고 자신과 source node로부터 SPD가 가까운 이웃 노드에 대한 confidence는 delta로 근사한다.
% 자신보다 source node로부터 SPD가 먼 이웃에 대한 confidence는 detla^2로 근사한다.
% 즉, 자기 자신과의 상대적 SPD from source nodes 우위를 비교하여, 그 값 클 수록 더 작은 값의 근사된 confidence를 할당한다.
% first step인 Diffusion 과 second step인 update 과정에 모두 관여하는 이 근사 방법은 CBFR에게 매우 중요한 요소이다. 

==> previous_version/3.4-1.tex <==
\subsection{EC-Based Feature Diffusion}
\label{sub:ecfd}

In this section, we present EC-based feature diffusion which is a first stage of CBFR.

% Diffusion is a process that consists of iterative propagation, which can be expressed as iteratively multiplying a feature matrix by a transition matrix.

To estimate missing node features via diffusion, source nodes propagate their features to their neighbors for each channel independently. While source nodes keep their features that are true values, missing nodes aggregate features from connected nodes. Missing nodes aggregate inaccurate tentative features from other connected missing nodes in addition to features from source nodes. Built on confidence which is an essential concept for missing features setting, We design a novel transition matrix for feature diffusion. Our design objective is that a missing node aggregate more features from node features with high EC. To this end, we consider EC in features for neighboring nodes of a specific missing feature.

Suppose a missing node feature $x_{i,d}$ of $v_i$ aggregates features from $v_j \in \mathcal{N}(v_i)$. We observe that difference between SPDFS of $v_i$ and SPDFS of $v_j$ cannot exceed 1. Formally, This observation can be expressed as the following theorem with proof in Appendix. 
\newtheorem{theorem}
\label{theorem1}
\begin{theorem}
Given a node $v_i$ s.t. $s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})=m\geq1$. Then, $s(v_j|\mathcal{V}^{(d)}_k, A^{(d)}) \in \{m-1,m,m+1\}$ for $v_j \in \mathcal{N}(v_i).$ Otherwise, if $v_i$ s.t. $s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})=0$ is given, $s(v_j|\mathcal{V}^{(d)}_k, A^{(d)}) \in \{0,1\}$ for $v_j \in \mathcal{N}(v_i).$
\end{theorem}
From Theorem 1, the following corollary holds trivially.

\begin{corollary}
If $s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})=m\geq1$, then \ $s(v_j|\mathcal{V}^{(d)}_k, A^{(d)})-s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})  \in \{-1,0,1\}$ for $v_j \in \mathcal{N}(v_i)$. Otherwise, if $s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})=0$, then $s(v_j|\mathcal{V}^{(d)}_k, A^{(d)})-s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})  \in \{0,1\}$ for $v_j \in \mathcal{N}(v_i)$.
\end{corollary}

Theorem 1 shows that from any node, there are at most three possible cases for SPDFS of its neighbors. Further, Collorary 1. shows that when moving to a nieghboring node, there are at most three possible changes in SPDFS. We then define relative EC $\hat{\rho}_{r}$, a function to output relative amount of EC in a particular node feature compared to other node features as follows
\newtheorem{definition5}{Definition}
\label{definition5}
\begin{definition}
Relative EC in $\bar{x}_{j,d}$ to $\bar{x}_{i,d}$ is define by $\hat{\rho}_{r} (\bar{x}_{j,d}| \bar{x}_{i,d}) = \hat{\rho}(\bar{x}_{j,d}|\mathcal{V}^{d}_k , A^{(d)}) / \hat{\rho}(\bar{x}_{i,d}|\mathcal{V}^{d}_k , A^{(d)})$.
\end{definition}

By Definition 4, we can rewrite $\hat{\rho}_{r} (\bar{x}_{j,d}| \bar{x}_{i,d})$ as $\alpha^{s(v_j|\mathcal{V}^{(d)}_k, A^{(d)})-s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})}$. Then, according to Corollary 1, the following corollary also holds.


\begin{corollary}
If $s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})=m\geq1$, then $\hat{\rho}_{r} (\bar{x}_{j,d}| \bar{x}_{i,d}) \in \{\alpha^{-1}, 1, \alpha\}\,$ for $v_j \in \mathcal{N}(v_i)$. Otherwise, if $s(v_i|\mathcal{V}^{(d)}_k, A^{(d)})=0$, then $\hat{\rho}_{r} (\bar{x}_{j,d}| \bar{x}_{i,d}) \in \{ 1, \alpha\}\,$ for $v_j \in \mathcal{N}(v_i)$.
\end{corollary}

Corollary 1.2 shows that at the point of view of a missing node, there are only three possible cases for relative EC in its neighboring feature to its feature, while two cases for a source node.

Before defining a transition matrix, we reorder nodes according to whether a feature value is known or not for $d$-channel, i.e., $x^{(d)}$ and $A^{(d)}$ are reordered for each channel as described in Section~\ref{problem_statement}. After the feature diffusion stage, we order the nodes according to the original numbering.

Let $\tilde{X}=[\tilde{x}_{i,d}]$ denote an estimate of full feature $X$, which is updated via propagation steps in EC-based feature diffusion. Built on Corollary 1.2, we construct a weighted adjacency matrix $W^{(d)}$ for $d$-th channel with $\alpha_1$ for a hyperparameter $\alpha$. $W^{(d)} \in \mathbb{R}^{N \times N}$ is defined as follows,
\begin{equation}
    W^{(d)}_{i,j} = \begin{cases} \hat{\rho}_{r} (\tilde{x}_{j,d}| \tilde{x}_{i,d}) & \,\text{if} \; i \neq j \, , \, A^{(d)}_{i,j} = 1
    \\
    0 & \,\text{if} \; i \neq j \, , \, A^{(d)}_{i,j} = 0
    \\
    1 & \,\text{if} \; i = j
    \end{cases}
\end{equation}
Note that self-loops are added to $W^{(d)}$ with weight 1 so that each node can keep some of its own feature.

$W^{d}_{i,j}$ is an edge weight corresponding to message passing from $v_j$ to $v_i$. According to Corollary 1.2, $W^{(d)}_{i,j} \in \{\alpha^{-1}, 0, \alpha\}$ when $v_i$ and $v_j$ are connected. Hence, $\alpha^{-1}$ is assigned as edge weights for high-EC neighbors while 1 for same-EC and $\alpha$ for low-EC neighbors. From a node's point point of view, $W^{d}$ allows node to aggregate more features with high EC from its neighbors. Furthermore, consider two connected nodes $v_i$ and $v_j$ s.t.  $\hat{\rho}_{r} (\bar{x}_{j,d}| \bar{x}_{i,d})=\alpha$. By Definition 5, $\hat{\rho}_{r} (\bar{x}_{i,d}| \bar{x}_{j,d}) = (\hat{\rho}_{r} (\bar{x}_{j,d}| \bar{x}_{i,d}))^{-1}$, so that $W^{(d)}_{i,j} = (W^{(d)}_{j,i})^{-1} = \alpha^{-1}$. This means that message passing from a high-EC node to a low-EC node occurs with large weight while message passing in the opposite direction occurs with small weight.

% 더욱이, EC가 다른 연결된 두 노드를 고려해보자.
% By Definition 5, $\hat{\rho}_{r} (\bar{x}_{i,d}| \bar{x}_{j,d}) = (\hat{\rho}_{r} (\bar{x}_{j,d}| \bar{x}_{i,d}))^{-1}$, i.e., $W^{(d)}_{i,j} = (W^{(d)}_{j,i})^{-1}$.
% 이는 EC가 높은 곳에서 적은 곳으로의 propagation은 많이 일어날 때, 낮은 곳에서 높은 곳으로의 propagation은 적게 일어나는 것을 의미한다.
% $W^{d}$ allows $\tilde{x}_{i,d}$ to aggregate more features with high EC from its neighbors.
%  A_ij는 node i가 node j로 부터 받아오는 것에 대응되는 edge weight를 의미한다. 따라서 두 노드의 AP(v_i)>AP(v_j)일 때, confidence가 더 높은 v_i는 v_j로 더 많은 feature를 전파할 수 있도록 한다 while v_i는 v_j로부터 적은 feature를 받아온다.
% 더욱이
% According to Corollary 1.2, $W^{(d)}_{i,j} \in \{\alpha^{-1}, 0, \alpha\}$ when $v_i$ and $v_j$ are connected. By Definition 5, $\hat{\rho}_{r} (\bar{x}_{i,d}| \bar{x}_{j,d}) = (\hat{\rho}_{r} (\bar{x}_{j,d}| \bar{x}_{i,d}))^{-1}$, i.e., $W^{(d)}_{i,j} = (W^{(d)}_{j,i})^{-1}$. 


% 추가


To ensure convergence of diffusion process, we then define $\hat{W}^{(d)} =(D^{(d)})^{-1} W^{(d)}$ through row-stochastic normalization with $D^{(d)}_{ii} = \Sigma_j W_{i,j}$.
Since $x^{d}_k$ with true feature values should be preserved, we replace first $|\mathcal{V}^{(d)}|$ rows of $\hat{W}$ with one-hot vectors indicating $\mathcal{V}^{(d)}_k$. A transition matrix $\tilde{W}$ for diffusion can be expressed as
\begin{equation}
    \tilde{W} = \begin{bmatrix}
\textbf{I} & \textbf{0} \\
\hat{W}^{(d)}_{uk} & \hat{W}^{(d)}_{uu}
\end{bmatrix}.
\end{equation}
Note that $\tilde{W}$ is still row-stochastic despite of the substitution of an identity matrix $\textbf{I}$ and a zero matrix $\textbf{0}$.
An aggregation in a specific node can be regarded as a weighted sum of features on neighboring nodes. A row-stochastic matrix for transition matrix means that when a node aggregates features from its neighbors, the sum of the weights is 1. Therefore, unlike symmetric or column-stochastic (random walk) transition matrix, features of missing nodes can be formed at the same scale of known features.

For diffusion, we initialize missing feature values $x^{(d)}_u$ to zero. Now, We define K-steps EC-based feature diffusion as
\begin{equation}
\begin{split}
   &\tilde{x}^{(d)} (t) = \tilde{W}\, \tilde{x}^{(d)} (t-1)\\&
\tilde{x}^{(d)} (K) = \tilde{W}^K \tilde{x}(0)
\end{split}
\end{equation}
where $\tilde{x}^{(d)} (t)$ denotes estimate of ${x}^{(d)}$ after t-steps diffusion.
% 평형점

% 다시 되돌려서 concatenate


==> previous_version/3.5-0.tex <==
 \subsection{Channel Correlation Propagation}
 \label{sub:fucc}
In the previous stage, We obtain $\tilde{X}$ (pre-estimate of $X$) via EC-based feature diffusion performed for each channel separately. The feature diffusion in based on graph structure and EC but not interdependence between channels. Since interdependence between channels can be an another important key for recovering missing node features, we propose a novel scheme to update $\tilde{X}$ by considering both channel correlation and EC.

We first prepare covariance matrix $C = [C_{a,b}]\in \mathbb{R}^{F \times F}$ giving the covariance between each pair of channels for the following proposed scheme. $C_{a,b}$, the covariance between $\tilde{X}_{:,a}$ and $\tilde{X}_{:,b}$ is calculated as
\begin{equation*}
    C_{a,b} = \frac{1}{N-1} \sum^N_{i=1} (\tilde{x}_{i,a} - m_a )(\tilde{x}_{i,b} - m_b)
\end{equation*}
where $m_d$ denote the mean of a graph signal for $d$-th channel, i.e., $m_d=\frac{1}{N}\sum^N_{i=1} \tilde{x}_{i,d}$.

In this stage, unlike looking across the nodes for each channel in the previous stage, we look across the channels for each node. We define weighted directed graphs $\{\mathcal{H}^{(i)}\}^N_{i=1}$ called Channel Correlation Graphs (CCGs) from the given graph $\mathcal{G}$. $\mathcal{H}^{(i)}$, CCG for a $i$-th node in $\mathcal{G}$ is defined as
\begin{equation}
\mathcal{H}^{(i)} = (\mathcal{V}^{(i)}, \mathcal{E}^{(i)}, B^{(i)})
\end{equation}
where $\mathcal{V}^{(i)}=\{v^{(i)}_d\}^F_{d=1}$ is a set of nodes in $\mathcal{H}^{(i)}$, $\mathcal{E}^{(i)}$ is a set of directed edges in $\mathcal{H}^{(i)}$, and $B^{(i)} \in \mathbb{R}^{F \times F}$ is a weighted undirected adjacency matrix to update $\tilde{X}_{i,:}$. To update $\tilde{x}_{i,d}$ of a $i$-th node via channel-wise propagation, we assign $\tilde{x}_{i,d}$ to each $v^{(i)}_d$ as a node feature for $d \in \{1, ..., F\}$. $\mathcal{E}^{(i)}$ is determined by $B^{(i)}$ which will be described.

Our design goals for $B^{(i)}$ are threefold: (1) To reflect correlation between channels via $C$, (2) To allow high-EC $\tilde{x}_{i,d}$ to propagate more feature, and (3) To update more for low-EC $\tilde{x}_{i,d}$. Based on these three design goals, we define $B^{(i)}$ as follows
\begin{equation}
\label{eq:matrixB}
B^{(i)}_{a,b} = \begin{cases} \gamma \, (1-\beta^{S_{i, a}}) \frac{1}{\sum^F_{b \neq a} \alpha^{S_{i, b}}} \sum^F_{b \neq a} \alpha^{S_{i, b}} C_{a,b}(\tilde{X}_{i,b} - m_b)& \;\text{if} \; a \neq b 
    
    \\
    1 & \;\text{if} \; a = b
    \end{cases}
\end{equation}
where $\beta$ is the additional hyperparameter used as $\alpha$ in Definition 3, $\gamma$ is the hyperparameter for scaling, and $m_b=\frac{1}{N}\sum^N_{i=1} \tilde{x}_{i,b}$. Self-loops in $B^{(i)}$ let each $v^{(i)}_d$ preserve pre-estimate $\tilde{x}_{i,d}$, while the other edges are involved in update. Note that $B^{(i)}_{a,b}$ is a weight of a directed edge corresponding to message passing to $v^{(i)}_a$ from $v^{(i)}_b$. In Eq (\ref{eq:matrixB}), $C_{a,b}(\tilde{X}_{i,b} - m_b)$,  $\alpha^{S_{i, b}}$, and $(1-\beta^{S_{i, b}})$ meet the design goal (1), (2), and (3), respectively.
% 베타는 EC.

Channel correlation propagation on $\mathcal{H}^{(i)}$ outputs $\hat{X}_{i,:}$, the final estimate of $X_{i,:}$:
\begin{equation}
\label{eq:Xhat}
\hat{X}_{i,:} = (B^{(i)} \tilde{X}^\top_{i,:})^\top
\end{equation}
Here, note that $\hat{X}_{i,:}$ and $\tilde{X}_{i,:}$ are row vectors. After calculating $\hat{X}_{i,:}$ for $i \in \{1, ...,N\}$, we obtain the final estimate by concatenating them, i.e., $\tilde{X} = [{\tilde{X}_{1, :}}^\top\; {\tilde{X}_{2, :}}^\top \;\, \cdots \;\, {\tilde{X}_{N, :}}^\top]^\top$. Moreover, since $C$ is calculated via pre-estimated features for all nodes in $\mathcal{G}$, channel correlation propagation injects global information into estimate of $X$. $\hat{X}$ is a final output of EC-based feature recovery (ECFR) and is fed to GNN to solve a downstream task.

% X hat which is the final estimate of X은 다음과 같이 얻어진다.
% 우리는 Xtilde을 업데이트 하여 Xhat을 얻는다.
% 이 과정이 Channel-wise Propagation
% 채널마다 그래프를 생성.
% 채널마다 수행한 후.
% concatenate.


% global information을 담고 있다.


% N개의 노드에 대해서 생성

% 이에 맞추어 3.2도 바꿀 것.

%  채널들간의 covariance를 계산하여 covariance matrix를 정의한다.
% C는 모든 노드들에 대하여 계산.
%  global information이 녹아있다.

% 이번 단계에서는, 각 채널마다 노드들을 가로질러서 보는 게 아니라. 노드마다 채널을 가로질러서 본다.
% 채널 방향의 directed graph를 각 노드마다 정의한다. 그것에 대한 수식 표현.
% 그리고 그 directed graph의 adjacency matrix에 해당하는 것은 이와 같다.
% equation
%  where ... .

% 
 
%  딱 두 가지.





% 그래프를 생성한다.

%  global information
%  across the channel 로 계산을 하나 global information이 녹아있다.

% relation, dependency
% 다시 리셋

% 3.3 설명도 바꿀까? 새로운 그래프를 만드는 것으로?

==> previous_version/3.5-1.tex <==
 \subsection{Node-wise Between-channel Propagation}
 \label{sub:ccp}
In the previous stage, we obtain $\tilde{X}=[\tilde{x}_{i,d}]$ (pre-recovered features for $X$) via Channel-wise between-node feature diffusion performed for each channel separately. The proposed feature diffusion is done based on graph structure and pseudo-confidence, but does not consider dependency between channels. Since the dependency between channels can be another important factor for recovering missing node features, we develop an additional scheme to update $\tilde{X}$ by considering both channel correlation and pseudo-confidence.

We first prepare covariance matrix $C = [C_{a,b}]\in \mathbb{R}^{F \times F}$ giving the covariance between each pair of channels for the following proposed scheme. $C_{a,b}$, the covariance between $\tilde{X}_{:,a}$ and $\tilde{X}_{:,b}$ is calculated as
\begin{equation}
    C_{a,b} = \frac{1}{N-1} \sum^N_{i=1} (\tilde{x}_{i,a} - m_a )(\tilde{x}_{i,b} - m_b)
\end{equation}
where $m_d$ denotes the mean of a graph signal for $d$-th channel, i.e., $m_d=\frac{1}{N}\sum^N_{i=1} \tilde{x}_{i,d}$.

In this stage, unlike looking across the nodes for each channel in the previous stage, we look across the channels for each node. As shown in the right hand graph of Figure~\ref{fig:framework}, we define directed graphs $\{\mathcal{H}^{(i)}\}^N_{i=1}$ called Node-wise Between-channel Propagation (NwBcP) graphs from the given graph $\mathcal{G}$. $\mathcal{H}^{(i)}$ for a $i$-th node in $\mathcal{G}$ is defined as
\begin{equation}
\mathcal{H}^{(i)} = (\mathcal{V}^{(i)}, \mathcal{E}^{(i)}, B^{(i)})
\end{equation}
where $\mathcal{V}^{(i)}=\{v^{(i)}_d\}^F_{d=1}$ is a set of nodes in $\mathcal{H}^{(i)}$, $\mathcal{E}^{(i)}$ is a set of directed edges in $\mathcal{H}^{(i)}$, and $B^{(i)} \in \mathbb{R}^{F \times F}$ is a weighted adjacency matrix to update $\tilde{X}_{i,:}$. To update $\tilde{x}_{i,d}$ of a $i$-th node via between-channel propagation, we assign $\tilde{x}_{i,d}$ to each $v^{(i)}_d$ as a node feature for a $d$-th channel ($d\in\{ 1, ..., F\}$). The weights in $\mathcal{E}^{(i)}$ are given by $B^{(i)}$ which will be described.

Our design goals of $B^{(i)}$ for  between-channel propagation in each node are to achieve threefold: (1) highly correlated channels should exchange more information to each other than less correlated channels, (2) high PC channel feature should propagate more information to other channels of the node than low PC channel feature, and (3) low PC channel feature should receive more information from other channels for recovery than high PC channel feature.
Based on these three design goals, 
the weight of the directed edge from $b$ channel to $a$ channel ($B^{(i)}_{a,b}$) in $B^{(i)}$ 
is designed by  
%we define $B^{(i)}$ as follows
\begin{equation}
\label{eq:matrixB}
B^{(i)}_{a,b} = \begin{cases} \gamma \, (1-\alpha '^{S_{i, a}}) \frac{1}{\sum^F_{b' \neq a}
\alpha^{S_{i, b'}}} %\sum^F_{b \neq a}
\alpha^{S_{i, b}} C_{a,b}(\tilde{x}_{i,b} - m_b)& \;\text{if} \; a \neq b 
    
    \\
    1 & \;\text{if} \; a = b
    \end{cases},
\end{equation}
where $C_{a,b}(\tilde{x}_{i,b} - m_b)$,  $\alpha^{S_{i, b}}$, and $(1-\beta^{S_{i, a}})$ are terms to meet the design goal (1), (2), and (3), respectively.
$\beta$ is  additional hyperparameter used along with $\alpha$ in Definition 3, and $\gamma$ is the scaling hyperparameter.
%, and $m_b=\frac{1}{N}\sum^N_{i=1} \tilde{x}_{i,b}$.
The self-loop weight $B_{d,d}^{(i)}$ derives each $v^{(i)}_d$ to preserve pre-recovered features $\tilde{x}_{i,d}$, while the other edge weights contribute to channel feature updates. 
%Note that $B^{(i)}_{a,b}$ is a weight of a directed edge corresponding to message passing to $v^{(i)}_a$ from $v^{(i)}_b$. In Eq (\ref{eq:matrixB}), $C_{a,b}(\tilde{x}_{i,b} - m_b)$,  $\alpha^{S_{i, b}}$, and $(1-\beta^{S_{i, b}})$ meet the design goal (1), (2), and (3), respectively.

Node-wise propagation on $\mathcal{H}^{(i)}$ outputs the final recovered features for $X_{i,:}$. Hence $i$-th row vector of $\hat{X}$, i.e.$\hat{X}_{i,:}$ becomes
\begin{equation}
\label{eq:Xhat}
\hat{X}_{i,:} = (B^{(i)} \tilde{X}^\top_{i,:})^\top,
\end{equation}
where $\hat{X}_{i,:}$ and $\tilde{X}_{i,:}$ are row vectors. After calculating $\hat{X}_{i,:}$ for $i \in \{1, ...,N\}$, we obtain the final recovered features by concatenating them, i.e., $\hat{X} = [{\hat{X}_{1, :}}^\top\; {\hat{X}_{2, :}}^\top \;\, \cdots \;\, {\hat{X}_{N, :}}^\top]^\top$. Moreover, since $C$ is calculated via pre-recovered features $\tilde{X}$ for all nodes in $\mathcal{G}$, channel correlation propagation injects global information into recovered features for $X$. $\hat{X}$ is a final output of PC-based feature recovery (PCFR) and is fed to GNN to solve a downstream task.

==> tables/ablation_table.tex <==
\begin{table}[h!]
\rv{
\caption{Ablation study of PCFR. row-ST, CGD and, NIP denote a row-stochastic transition matrix, channel-wise graph diffusion, and node-wise inter-channel propagation, respectively.}
\centering
\scriptsize
\label{ablation_table}
% \renewcommand{\arraystretch}{0.7}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccc|cccc}
\hline
\multicolumn{4}{c|}{Cora}                                                           & \multicolumn{4}{c}{CiteSeer}                                                       \\ \hline
row-ST      & CGD       & \multicolumn{1}{c|}{NIP}    & \multicolumn{1}{c|}{accuracy (\%)} & row-ST      & CGD       & \multicolumn{1}{c|}{NIP}    & \multicolumn{1}{c}{accuracy (\%)} \\ \hline
{\textcolor{red}{\ding{55}}} & {\textcolor{red}{\ding{55}}} & \multicolumn{1}{c|}{\textcolor{red}{\ding{55}}} & $73.57 \pm 2.61$                    & {\textcolor{red}{\ding{55}}} & {\textcolor{red}{\ding{55}}} & \multicolumn{1}{c|}{\textcolor{red}{\ding{55}}} & $56.98 \pm 3.48$                   \\
{\textcolor{green}{\ding{51}}} & {\textcolor{red}{\ding{55}}} & \multicolumn{1}{c|}{\textcolor{red}{\ding{55}}} & $75.12 \pm 2.15$                    & {\textcolor{green}{\ding{51}}} & {\textcolor{red}{\ding{55}}} & \multicolumn{1}{c|}{\textcolor{red}{\ding{55}}} & $62.00 \pm 3.28$                   \\
{\textcolor{green}{\ding{51}}} & {\textcolor{green}{\ding{51}}} & \multicolumn{1}{c|}{\textcolor{red}{\ding{55}}} & $75.47 \pm 1.51$                    & {\textcolor{green}{\ding{51}}} & {\textcolor{green}{\ding{51}}} & \multicolumn{1}{c|}{\textcolor{red}{\ding{55}}} & $63.08 \pm 1.73$                   \\
{\textcolor{green}{\ding{51}}} & {\textcolor{red}{\ding{55}}} & \multicolumn{1}{c|}{\textcolor{green}{\ding{51}}} & $75.32 \pm 1.89$                    & {\textcolor{green}{\ding{51}}} & {\textcolor{red}{\ding{55}}} & \multicolumn{1}{c|}{\textcolor{green}{\ding{51}}} & $62.32 \pm 2.88$
\\
{\textcolor{green}{\ding{51}}} & {\textcolor{green}{\ding{51}}} & \multicolumn{1}{c|}{\textcolor{green}{\ding{51}}} & $\mathbf{76.00\pm1.22}$                    & {\textcolor{green}{\ding{51}}} & {\textcolor{green}{\ding{51}}} & \multicolumn{1}{c|}{\textcolor{green}{\ding{51}}} & $\mathbf{63.82\pm1.78}$
\\ \hline
\end{tabular}
}
}
\end{table}

==> tables/hyperparam_table.tex <==
\begin{table}[h!]
\caption{Hyperparameters of PCFR used in node classification.}
\centering
\scriptsize
\label{hyperparam_table}
% \renewcommand{\arraystretch}{0.7}
{\small
\begin{tabular}{cc|ccc|ccc}
\hline
\multicolumn{2}{c|}{Missing type}                            & \multicolumn{3}{c|}{Structural missing} & \multicolumn{3}{c}{Uniform missing} \\ \hline
\multicolumn{2}{c|}{$r_m$}                                   & 0.995       & 0.9         & 0.5         & 0.995      & 0.9        & 0.5       \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{Cora}}       & $\alpha$  & 0.8         & 0.9         & 0.9         & 0.8        & 0.9        & 0.9       \\
\multicolumn{1}{c|}{}                            & $\alpha'$ & 0.4         & 0.4         & 0.2         & 0.4        & 0.3        & 0.3       \\
\multicolumn{1}{c|}{}                            & $\gamma$  & $10^3$      & $10^2$      & $10^2$      & 10         & 1          & 1         \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{CiteSeer}}   & $\alpha$  & 0.8         & 0.8         & 0.8         & 0.8        & 0.8        & 0.8       \\
\multicolumn{1}{c|}{}                            & $\alpha'$ & 0.3         & 0.3         & 0.4         & 0.3        & 0.3        & 0.3       \\
\multicolumn{1}{c|}{}                            & $\gamma$  & $10^3$      & $10^3$      & $10^3$      & $10^4$     & $10^4$     & $10^4$    \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{PubMed}}     & $\alpha$  & 0.9         & 0.9         & 0.7         & 0.6        & 0.9        & 0.9       \\
\multicolumn{1}{c|}{}                            & $\alpha'$ & 0.2         & 0.2         & 0.5         & 0.7        & 0.5        & 0.3       \\
\multicolumn{1}{c|}{}                            & $\gamma$  & $10^6$      & $10^6$      & $10^6$      & $10^4$     & $10^7$     & $10^7$    \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{Photo}}      & $\alpha$  & 0.6         & 0.4         & 0.8         & 0.6        & 0.6        & 0.6       \\
\multicolumn{1}{c|}{}                            & $\alpha'$ & 0.7         & 0.7         & 0.7         & 0.7        & 0.7        & 0.7       \\
\multicolumn{1}{c|}{}                            & $\gamma$  & $10^2$      & 10          & 10          & 10         & 1          & 1         \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{Computers}}  & $\alpha$  & 0.8         & 0.4         & 0.1         & 0.4        & 0.4        & 0.4       \\
\multicolumn{1}{c|}{}                            & $\alpha'$ & 0.4         & 0.4         & 0.4         & 0.7        & 0.7        & 0.7       \\
\multicolumn{1}{c|}{}                            & $\gamma$  & $10^3$      & $10^3$      & $10^2$      & $10^2$     & $10^2$     & $10^3$    \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{OGBN-Arxiv}} & $\alpha$  & 0.3         & 0.3         & 0.1         & 0.7        & 0.7        & 0.7       \\
\multicolumn{1}{c|}{}                            & $\alpha'$ & 0.7         & 0.7         & 0.7         & 0.3        & 0.3        & 0.3       \\
\multicolumn{1}{c|}{}                            & $\gamma$  & $10^5$      & $10^5$      & $10^5$      & $10^6$     & $10^6$     & $10^5$    \\ \hline
\end{tabular}
}
\end{table}

==> tables/imbalacned_table.tex <==
\begin{table}[h!]
\caption{\rv{Class-imbalanced node classification accuracy (\%) at a missing rate $r_m=0.995$. OOM denotes out of memory. * denotes incalculable average for 5 datasets due to OOM results.}}
\centering
\label{tab: imbalance}
\rv{
\resizebox{\textwidth}{!}{
\begin{tabular}{l|l|cccccc}
\toprule
Missing type                                                                  & Dataset   & \multicolumn{1}{c}{sRMGCNN} & \multicolumn{1}{c}{GCNMF} & \multicolumn{1}{c}{PaGNN} & \multicolumn{1}{c}{LP} & \multicolumn{1}{c}{FP} & \multicolumn{1}{c}{PCFR} \\ \midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}Structural\\ missing\end{tabular}} 
                      & Cora    & $29.29\pm0.71$   
                                & $32.98\pm3.35$             
                                & $46.93\pm6.43$          
                                & $75.78\pm1.85$           
                                & $73.85\pm1.90$          
                                & $\mathbf{76.05\pm2.38}$  \\
                     & CiteSeer & $24.33\pm1.15$  
                                & $24.89\pm1.78$             
                                & $34.10\pm4.68$            
                                & $67.02\pm3.33$            
                                & $63.69\pm2.36$          
                                & $\mathbf{67.31\pm1.77}$  \\
                    & PubMed    & OOM 
                                & $40.06\pm0.60$
                                & $53.65\pm3.28$       
                                & $70.53\pm3.30$           
                                & $72.01\pm3.55$         
                                & $\mathbf{73.31\pm3.22}$  \\
                    & Photo     & $29.25\pm3.43$    
                                & $29.15\pm3.03$            
                                & $82.49\pm1.68$            
                                & $84.27\pm2.11$            
                                & $87.45\pm0.98$         
                                & $\mathbf{87.54\pm1.06}$  \\
                    & Computers & $37.15\pm0.12$  
                                & $37.11\pm0.16$             
                                & $75.63\pm1.71$            
                                & $77.67\pm2.02$            
                                & $79.03\pm1.59$      
                                & $\mathbf{79.86\pm1.28}$  \\
                 \cmidrule{2-8}                                            
                 & Average      & \multicolumn{1}{c}{*}        
                                & \multicolumn{1}{c}{32.84} 
                                & \multicolumn{1}{c}{58.56} 
                                & \multicolumn{1}{c}{75.05} 
                                & \multicolumn{1}{c}{75.21} 
                                & \multicolumn{1}{c}{$\mathbf{76.81}$} \\
\midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ missing\end{tabular}} 
                      & Cora    & $29.29\pm0.71$   
                                & $30.72\pm1.46$             
                                & $65.11\pm2.65$            
                                & $75.78\pm1.85$           
                                & $77.31\pm1.16$          
                                & $\mathbf{78.39\pm0.77}$  \\
                     & CiteSeer & $23.76\pm1.80$  
                                & $27.63\pm3.08$             
                                & $57.63\pm2.80$            
                                & $67.02\pm3.33$            
                                & $68.52\pm1.73$          
                                & $\mathbf{69.42\pm2.49}$  \\
                    & PubMed    & OOM  
                                & $40.14\pm0.60$       
                                & $58.92\pm2.25$            
                                & $70.53\pm3.30$           
                                & $72.12\pm3.77$         
                                & $\mathbf{74.67\pm3.07}$  \\
                    & Photo     & $28.67\pm2.95$    
                                & $33.43\pm8.62$            
                                & $87.62\pm1.42$            
                                & $84.27\pm2.11$            
                                & $88.56\pm0.96$         
                                & $\mathbf{88.69\pm1.09}$  \\
                    & Computers & $37.13\pm0.10$  
                                & $37.15\pm0.12$             
                                & $82.85\pm1.40$            
                                & $77.67\pm2.02$            
                                & $82.99\pm1.47$         
                                & $\mathbf{83.87\pm1.21}$  \\
                 \cmidrule{2-8}                                            
                 & Average      & \multicolumn{1}{c}{*}        
                                & \multicolumn{1}{c}{33.81} 
                                & \multicolumn{1}{c}{70.43} 
                                & \multicolumn{1}{c}{75.05} 
                                & \multicolumn{1}{c}{77.90} 
                                & \multicolumn{1}{c}{$\mathbf{79.01}$} \\                             \bottomrule
\end{tabular}
}
}
\end{table}


==> tables/link_pre_table.tex <==
\begin{table}[t]
\centering
\label{link_pre_table}
\caption{\rv{Link prediction results at missing rate $r_m =0.995$. OOM denotes out of memory.}}
\footnotesize
\rv{
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{ll|c|ccc|ccc}
\hline
                                                &     & Full-feature   & \multicolumn{3}{c|}{Structural missing}                   & \multicolumn{3}{c}{Uniform missing}                       \\ \cline{3-9} 
                                                &     &                & sRMGCNN        & FP             & PCFR                    & sRMGCNN        & FP             & PCFR                    \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{Cora}}      & AUC & $92.05\pm0.72$ & $68.17\pm1.11$ & $83.72\pm1.15$ & $\mathbf{84.42\pm0.95}$ & $66.45\pm5.63$ & $86.36\pm1.38$ & $\mathbf{86.88\pm1.32}$ \\
\multicolumn{1}{l|}{}                           & AP  & $92.59\pm0.87$ & $71.02\pm0.92$ & $86.11\pm1.08$ & $\mathbf{86.65\pm1.15}$ & $68.87\pm6.36$ & $88.72\pm1.09$ & $\mathbf{88.93\pm1.24}$ \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{CiteSeer}}  & AUC & $90.46\pm0.98$ & $67.77\pm1.95$ & $79.31\pm1.46$ & $\mathbf{80.25\pm2.13}$ & $64.65\pm5.19$ & $81.49\pm2.24$ & $\mathbf{82.06\pm2.14}$ \\
\multicolumn{1}{l|}{}                           & AP  & $91.52\pm1.04$ & $69.09\pm1.88$ & $82.99\pm1.37$ & $\mathbf{83.83\pm1.52}$ & $66.30\pm5.65$ & $85.89\pm1.72$ & $\mathbf{86.01\pm1.67}$ \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{PubMed}}    & AUC & $91.61\pm0.47$ & OOM            & $78.47\pm1.95$ & $\mathbf{79.66\pm0.85}$ & OOM            & $76.92\pm3.78$ & $\mathbf{80.65\pm0.98}$ \\
\multicolumn{1}{l|}{}                           & AP  & $92.03\pm0.40$ & OOM            & $84.05\pm1.16$ & $\mathbf{84.42\pm0.53}$ & OOM            & $83.12\pm2.38$ & $\mathbf{85.01\pm0.51}$ \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{Photo}}     & AUC & $95.75\pm0.45$ & $81.48\pm0.29$ & $94.13\pm1.16$ & $\mathbf{94.47\pm1.19}$ & $81.53\pm0.27$ & $93.81\pm2.30$ & $\mathbf{95.40\pm0.23}$ \\
\multicolumn{1}{l|}{}                           & AP  & $95.32\pm0.48$ & $81.07\pm0.33$ & $93.63\pm1.04$ & $\mathbf{93.78\pm1.15}$ & $81.14\pm0.29$ & $93.22\pm2.34$ & $\mathbf{94.78\pm0.27}$ \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{Computers}} & AUC & $93.77\pm1.11$ & $83.37\pm0.17$ & $90.62\pm1.22$ & $\mathbf{92.89\pm0.78}$ & $83.39\pm0.18$ & $90.12\pm2.54$ & $\mathbf{93.45\pm0.73}$ \\
\multicolumn{1}{l|}{}                           & AP  & $93.77\pm1.05$ & $83.66\pm0.24$ & $90.97\pm1.05$ & $\mathbf{92.70\pm0.95}$ & $83.68\pm0.26$ & $90.51\pm2.18$ & $\mathbf{93.47\pm0.67}$ \\ \hline
\end{tabular}
}
}
\label{tab:lp}
\end{table}
\vspace{-0.5mm}

==> tables/notation_table.tex <==
\begin{table}[h!]

\caption{Summary of notations in the paper.}

\centering
\label{notation_table}
% \renewcommand{\arraystretch}{0.7}
{{\footnotesize
\begin{tabular}{ll|ll}
\toprule
Symbol    & Description & Symbol     & Description \\ 
\midrule
$v_i$         & $i$-th node       
& $\mathcal{V}^{(d)}_k$        & set of known nodes in the $d$-th channel          \\
$\mathcal{N}(v_i)$   & neighboring nodes of $v_i$            
& $\mathcal{V}^{(d)}_u$         & set of unknown nodes in the $d$-th channel          \\
$\mX$     & full feature matrix       
& $x^{(d)}$         & graph signal for the $d$-th channel features        \\
$x_{i,d}$       & $d$-th channel feature of $v_i$        
& $x^{(d)}_k$        & $d$-th channel features for $\mathcal{V}^{d}_k$          \\
$\hat{\mX}$       & recovered feature matrix         
& $x^{(d)}_u$          & $d$-th channel features for $\mathcal{V}^{d}_u$          \\
$\hat{x}_{i,d}$       & $d$-th channel recovered feature of $v_i$            
& $\mA^{(d)}$         & reordered $A$ for the $d$-th channel          \\
\bottomrule
\end{tabular}}}
\end{table}

==> tables/sota_table.tex <==
\begin{table}[t]
\caption{Node classification accuracy (\%) at missing rate $r_m =0.995$. OOM denotes out of memory. * denotes incalculable average for 6 datasets due to OOM results.}
\centering
\label{sota_table}
% \renewcommand{\arraystretch}{0.7}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|l|ccccccc}
\toprule
Missing type                                                                  & Dataset   & \multicolumn{1}{c}{Baseline 1} & \multicolumn{1}{c}{Baseline 2 (LP)~\cite{zhu2002learning}} & \multicolumn{1}{c}{sRMGCNN~\cite{monti2017geometric}} & \multicolumn{1}{c}{GCNMF~\cite{taguchi2021graph}} & \multicolumn{1}{c}{PaGNN~\cite{jiang2020incomplete}} & \multicolumn{1}{c}{FP~\cite{rossi2021unreasonable}} & \multicolumn{1}{c}{PCFR} \\ \midrule
\multirow{7}{*}{\begin{tabular}[c]{@{}l@{}}Structural\\ missing\end{tabular}} & Cora    & $43.40\pm8.75$   & $74.10\pm1.25$             & $25.96\pm4.53$            & $31.77\pm2.37$           & $44.47\pm8.87$          & $73.57\pm2.61$         & $\mathbf{75.58\pm2.04}$  \\
                                                                              & CiteSeer & $29.18\pm2.73$  & $61.68\pm1.70$             & $22.97\pm0.52$            & $24.23\pm2.85$            & $30.40\pm3.25$          & $56.98\pm3.48$         & $\mathbf{63.45\pm2.17}$  \\
                                                                              & PubMed  & $49.53\pm4.13$    & $72.02\pm2.90$                        & OOM            & $40.39\pm0.62$            & $51.84\pm3.18$         & $73.38\pm2.85$         & $\mathbf{74.40\pm2.52}$  \\
                                                                              & Photo   & $78.96\pm3.08$   & $83.53\pm4.25$             & $24.02\pm3.52$            & $25.16\pm1.51$            & $80.85\pm3.26$         & $86.54\pm0.80$         & $\mathbf{86.93\pm0.94}$  \\
                                                                              & Computers & $70.07\pm2.85$  & $75.10\pm1.82$             & $36.38\pm1.30$            & $21.16\pm10.45$            & $72.52\pm2.11$         &    $77.40\pm1.70$      & $\mathbf{77.51\pm2.19}$  \\
                                                                              & OGBN-Arxiv& $49.23\pm1.16$ & $\mathbf{67.56\pm0.00}$                        & OOM                       & OOM            & $54.50\pm0.48$         & $65.85\pm0.44$         & $66.10\pm0.28$  \\ \cmidrule{2-9} 
                                                                              & Average    & \multicolumn{1}{c}{$53.40$}        & \multicolumn{1}{c}{$72.48$} & \multicolumn{1}{c}{*} & \multicolumn{1}{c}{*} & \multicolumn{1}{c}{$55.76$} & \multicolumn{1}{c}{$72.29$} & \multicolumn{1}{c}{$\mathbf{74.00}$}\\
                                                                              
                                                                              
                                                                              \midrule
\multirow{7}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ missing\end{tabular}}    & Cora  & $63.53\pm4.08$     & $74.10\pm1.25$             & $27.05\pm5.62$            & $25.21\pm7.42$            & $65.91\pm4.01$         & $78.15\pm1.03$         & $\mathbf{78.72\pm1.55}$  \\
                                                                              & CiteSeer & $50.97\pm2.59$  & $61.68\pm1.70$             & $23.23\pm0.00$            & $25.98\pm5.30$            & $51.89\pm2.52$         &  $65.63\pm1.08$        & $\mathbf{66.68\pm1.10}$  \\
                                                                              & PubMed   & $55.58\pm2.95$  & $72.02\pm2.90$                        & OOM            & $39.57\pm0.49$            & $61.12\pm3.87$         &    $74.19\pm2.91$      & $\mathbf{76.22\pm2.82}$  \\
                                                                              & Photo    & $84.46\pm1.76$  & $83.53\pm4.25$             & $24.86\pm1.54$            & $24.16\pm1.65$            & $86.75\pm1.19$          & $87.76\pm1.78$        & $\mathbf{88.08\pm1.62}$  \\
                                                                              & Computers & $78.38\pm1.51$  & $75.10\pm1.82$             & $33.37\pm6.29$            & $26.45\pm9.34$            & $79.92\pm1.71$         & $80.35\pm2.08$         & $\mathbf{80.47\pm1.74}$  \\
                                                                              & OGBN-Arxiv & $48.87\pm0.59$ & $\mathbf{67.56\pm0.00}$                        & OOM                       & OOM            & $58.91\pm0.41$         &    $63.90\pm0.42$      & $66.00\pm0.32$  \\ 
                                            \cmidrule{2-9} 
                                                                              & Average    & \multicolumn{1}{c}{$63.63$}        & \multicolumn{1}{c}{$72.48$} & \multicolumn{1}{c}{*} & \multicolumn{1}{c}{*} & \multicolumn{1}{c}{$67.42$} & \multicolumn{1}{c}{$75.00$} & \multicolumn{1}{c}{$\mathbf{76.03}$}\\                                  \bottomrule
\end{tabular}
}
\end{table}
\vspace{-0.5mm}

==> tables/sota_table_50.tex <==
\begin{table}[h!]
\caption{Node classification accuracy (\%) at missing rate $r_m =0.5$. OOM denotes out of memory. * denotes incalculable average for 6 datasets due to OOM results.}
\centering
\label{sota_table_50}
% \renewcommand{\arraystretch}{0.7}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|l|ccccccc}
\toprule
Missing type                                                                  & Dataset   & \multicolumn{1}{c}{Baseline 1} & \multicolumn{1}{c}{Baseline 2 (LP)~\cite{zhu2002learning}} & \multicolumn{1}{c}{sRMGCNN~\cite{monti2017geometric}} & \multicolumn{1}{c}{GCNMF~\cite{taguchi2021graph}} & \multicolumn{1}{c}{PaGNN~\cite{jiang2020incomplete}} & \multicolumn{1}{c}{FP~\cite{rossi2021unreasonable}} & \multicolumn{1}{c}{PCFR} \\ \midrule
\multirow{7}{*}{\begin{tabular}[c]{@{}l@{}}Structural\\ missing\end{tabular}} & Cora    & $79.10\pm1.28$   & $74.10\pm1.25$             & $43.82\pm4.16$            & $78.13\pm1.88$           & $79.53\pm1.38$          & $\mathbf{80.78\pm1.36}$         & $80.72\pm1.38$  \\
                                                                              & CiteSeer & $66.23\pm1.29$  & $61.68\pm1.70$             & $38.71\pm3.58$            & $65.06\pm1.36$            & $65.73\pm2.56$          & $66.37\pm2.03$         & $\mathbf{66.55\pm2.23}$  \\
                                                                              & PubMed  & $75.06\pm2.91$    & $72.02\pm2.90$                        & OOM            & $70.96\pm5.52$            & $75.22\pm3.12$         & $75.83\pm3.13$         & $\mathbf{77.57\pm3.07}$  \\
                                                                              & Photo   & $90.46\pm1.21$   & $83.53\pm4.25$             & $89.68\pm1.53$            & $88.10\pm2.93$            & $90.86\pm1.20$         & $90.47\pm0.94$         & $\mathbf{90.81\pm0.85}$  \\
                                                                              & Computers & $83.99\pm1.46$  & $75.10\pm1.82$             & $80.36\pm1.99$            & $76.63\pm7.12$            & $83.91\pm1.38$         &    $83.84\pm1.92$      & $\mathbf{83.85\pm1.32}$  \\
                                                                              & OGBN-Arxiv& $68.73\pm0.20$ & $67.56\pm0.00$                        & OOM                       & OOM            & $68.37\pm0.24$         & $\mathbf{69.29\pm0.17}$         & $69.25\pm0.20$  \\ \cmidrule{2-9} 
                                                                              & Average    & \multicolumn{1}{c}{$77.26$}        & \multicolumn{1}{c}{$72.48$} & \multicolumn{1}{c}{*} & \multicolumn{1}{c}{*} & \multicolumn{1}{c}{$77.27$} & \multicolumn{1}{c}{$77.76$} & \multicolumn{1}{c}{$\mathbf{78.13}$}\\
                                                                              
                                                                              
                                                                              \midrule
\multirow{7}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ missing\end{tabular}}    & Cora  & $80.02\pm1.42$     & $74.10\pm1.25$             & $62.74\pm5.59$            & $79.69\pm1.68$            & $80.21\pm1.74$         & $80.51\pm1.21$         & $\mathbf{80.54\pm1.18}$  \\
                                                                              & CiteSeer & $66.68\pm2.22$  & $61.68\pm1.70$             & $31.13\pm10.05$            & $65.89\pm1.27$            & $66.24\pm1.85$         &  $66.95\pm2.08$        & $\mathbf{69.21\pm1.96}$  \\
                                                                              & PubMed   & $75.85\pm3.00$  & $72.02\pm2.90$                        & OOM            & $75.40\pm2.10$            & $75.62\pm3.14$         &    $\mathbf{76.57\pm3.09}$      & $76.43\pm2.93$  \\
                                                                              & Photo    & $90.86\pm1.12$  & $83.53\pm4.25$             & $89.59\pm1.51$            & $79.77\pm6.91$            & $90.85\pm1.32$          & $\mathbf{91.14\pm0.71}$        & $90.99\pm1.21$  \\
                                                                              & Computers & $84.14\pm1.14$  & $75.10\pm1.82$             & $81.29\pm1.42$            & $68.69\pm12.00$            & $84.00\pm1.50$         & $83.73\pm1.60$         & $\mathbf{84.02\pm1.38}$  \\
                                                                              & OGBN-Arxiv & $68.28\pm0.18$ & $67.56\pm0.00$                        & OOM                       & OOM            & $68.54\pm0.16$         &    $69.32\pm0.24$      & $\mathbf{69.45\pm0.23}$  \\ 
                                            \cmidrule{2-9} 
                                                                              & Average    & \multicolumn{1}{c}{$77.64$}        & \multicolumn{1}{c}{$72.48$} & \multicolumn{1}{c}{*} & \multicolumn{1}{c}{*} & \multicolumn{1}{c}{$77.58$} & \multicolumn{1}{c}{$78.04$} & \multicolumn{1}{c}{$\mathbf{78.44}$}\\                                  \bottomrule
\end{tabular}
}
\end{table}
\vspace{-0.5mm}

==> tables/sota_table_90.tex <==
\begin{table}[h!]
\caption{Node classification accuracy (\%) at missing rate $r_m =0.9$. OOM denotes out of memory. * denotes incalculable average for 6 datasets due to OOM results.}
\centering
\label{sota_table_90}
% \renewcommand{\arraystretch}{0.7}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|l|ccccccc}
\toprule
Missing type                                                                  & Dataset   & \multicolumn{1}{c}{Baseline 1} & \multicolumn{1}{c}{Baseline 2 (LP)~\cite{zhu2002learning}} & \multicolumn{1}{c}{sRMGCNN~\cite{monti2017geometric}} & \multicolumn{1}{c}{GCNMF~\cite{taguchi2021graph}} & \multicolumn{1}{c}{PaGNN~\cite{jiang2020incomplete}} & \multicolumn{1}{c}{FP~\cite{rossi2021unreasonable}} & \multicolumn{1}{c}{PCFR} \\ \midrule
\multirow{7}{*}{\begin{tabular}[c]{@{}l@{}}Structural\\ missing\end{tabular}} & Cora    & $68.87\pm1.98$   & $74.10\pm1.25$             & $29.36\pm1.81$            & $69.45\pm1.80$           & $70.36\pm2.66$          & $79.16\pm1.49$         & $\mathbf{79.26\pm1.22}$  \\
                                                                              & CiteSeer & $54.35\pm2.62$  & $61.68\pm1.70$             & $23.16\pm0.45$            & $54.47\pm2.51$            & $55.31\pm2.41$          & $65.15\pm2.11$         & $\mathbf{65.29\pm1.26}$  \\
                                                                              & PubMed  & $67.92\pm2.89$    & $72.02\pm2.90$                        & OOM            & $44.95\pm5.18$            & $69.96\pm2.89$         & $75.71\pm2.92$         & $\mathbf{75.75\pm2.50}$  \\
                                                                              & Photo   & $88.53\pm1.34$   & $83.53\pm4.25$             & $27.03\pm1.90$            & $31.54\pm7.90$            & $89.41\pm0.86$         & $89.42\pm1.40$         & $\mathbf{89.75\pm1.06}$  \\
                                                                              & Computers & $81.82\pm1.27$  & $75.10\pm1.82$             & $35.26\pm3.80$            & $31.18\pm13.48$            & $82.34\pm1.13$         &    $81.20\pm1.44$      & $\mathbf{81.66\pm2.03}$  \\
                                                                              & OGBN-Arxiv& $64.10\pm0.37$ & $67.56\pm0.00$                        & OOM                       & OOM            & $64.65\pm0.40$         & $68.02\pm0.21$         & $\mathbf{68.03\pm0.25}$  \\ \cmidrule{2-9} 
                                                                              & Average    & \multicolumn{1}{c}{$70.93$}        & \multicolumn{1}{c}{$72.48$} & \multicolumn{1}{c}{*} & \multicolumn{1}{c}{*} & \multicolumn{1}{c}{$72.01$} & \multicolumn{1}{c}{$76.44$} & \multicolumn{1}{c}{$\mathbf{76.62}$}\\
                                                                              
                                                                              
                                                                              \midrule
\multirow{7}{*}{\begin{tabular}[c]{@{}l@{}}Uniform\\ missing\end{tabular}}    & Cora  & $72.44\pm1.57$     & $74.10\pm1.25$             & $25.69\pm5.24$            & $72.01\pm1.66$            & $75.34\pm1.63$         & $\mathbf{79.87\pm1.56}$         & $79.72\pm1.52$  \\
                                                                              & CiteSeer & $60.39\pm1.37$  & $61.68\pm1.70$             & $22.95\pm0.55$            & $57.97\pm2.13$            & $60.31\pm1.66$         &  $65.69\pm2.35$        & $\mathbf{68.23\pm1.62}$  \\
                                                                              & PubMed   & $69.22\pm3.37$  & $72.02\pm2.90$                        & OOM            & $63.01\pm4.40$            & $71.35\pm3.69$         &    $75.60\pm3.48$      & $\mathbf{75.91\pm3.45}$  \\
                                                                              & Photo    & $88.62\pm1.50$  & $83.53\pm4.25$             & $28.25\pm4.41$            & $30.65\pm9.40$            & $89.92\pm1.04$          & $89.54\pm1.25$        & $\mathbf{89.84\pm1.41}$  \\
                                                                              & Computers & $82.03\pm1.44$  & $75.10\pm1.82$             & $33.86\pm6.33$            & $30.29\pm9.68$            & $83.28\pm1.79$         & $81.87\pm1.41$         & $\mathbf{82.37\pm1.76}$  \\
                                                                              & OGBN-Arxiv & $63.82\pm0.32$ & $67.56\pm0.00$                        & OOM                       & OOM            & $65.58\pm0.22$         &    $68.15\pm0.24$      & $\mathbf{68.40\pm0.20}$  \\ 
                                            \cmidrule{2-9} 
                                                                              & Average    & \multicolumn{1}{c}{$72.75$}        & \multicolumn{1}{c}{$72.48$} & \multicolumn{1}{c}{*} & \multicolumn{1}{c}{*} & \multicolumn{1}{c}{$74.30$} & \multicolumn{1}{c}{$76.79$} & \multicolumn{1}{c}{$\mathbf{77.41}$}\\                                  \bottomrule
\end{tabular}
}
\end{table}
\vspace{-0.5mm}
